Provable Partially Observable Reinforcement Learning with Privileged Information

Partial observability of the underlying states generally presents significant challenges for reinforcement learning (RL). In practice, certain \emph{privileged information}, e.g., the access to states from simulators, has been exploited in training and has achieved prominent empirical successes. To better understand the benefits of privileged information, we revisit and examine several simple and practically used paradigms in this setting. Specifically, we first formalize the empirical paradigm of \emph{expert distillation} (also known as \emph{teacher-student} learning), demonstrating its pitfall in finding near-optimal policies. We then identify a condition of the partially observable environment, the \emph{deterministic filter condition}, under which expert distillation achieves sample and computational complexities that are \emph{both} polynomial. Furthermore, we investigate another useful empirical paradigm of \emph{asymmetric actor-critic}, and focus on the more challenging setting of observable partially observable Markov decision processes. We develop a belief-weighted asymmetric actor-critic algorithm with polynomial sample and quasi-polynomial computational complexities, in which one key component is a new provable oracle for learning belief states that preserve \emph{filter stability} under a misspecified model, which may be of independent interest. Finally, we also investigate the provable efficiency of partially observable multi-agent RL (MARL) with privileged information. We develop algorithms featuring \emph{centralized-training-with-decentralized-execution}, a popular framework in empirical MARL, with polynomial sample and (quasi-)polynomial computational complexities in both paradigms above. Compared with a few recent related theoretical studies, our focus is on understanding practically inspired algorithmic paradigms, without computationally intractable oracles.

==> Body/Formulation.tex <==
%!TEX root = main.tex
\newcommand{\cgk}{\overline{\cG}^k}
\newcommand{\ucgk}{\underline{\cG}^k}
\newcommand{\eecg}{\EE_{c_1}^{\cG}}
\newcommand{\eecgk}{\EE_{c_1}^{\cgk}}
\newcommand{\cpk}{\overline{\cP}^k}
\newcommand{\ucpk}{\underline{\cP}^k}
\newcommand{\eecp}{\EE_{c_1}^{\cP}}
\newcommand{\eecpk}{\EE_{c_1}^{\cpk}}
\newcommand{\cmk}{{\cM}^k}
\newcommand{\ucmk}{\underline{\cM}^k}
\newcommand{\eecm}{\EE_{c_1}^{\cM}}
\newcommand{\eecmk}{\EE_{c_1}^{\cmk}}
\newcommand{\trunc}{\text{trunc}}
\newcommand{\high}{\text{high}}
\newcommand{\low}{\text{low}}


\section{Learning observable POMDPs with asymmetric information}
\subsection{Preliminaries}
\paragraph{Model.}
Formally, we define a POMDP by a tuple $\cP = (H, \mathcal{S}, \mathcal{A}, \mathcal{O}, \mathbb{T}, \mathbb{O}, \mu_1, r)$, where $H$ denotes the length of each episode, $\mathcal{S}$ is the state space with $|\mathcal{S}|=S$, $\mathcal{A}$ denotes the action space with $|\mathcal{A}|=A$. We use $\mathbb{T}=\{\mathbb{T}_h\}_{h\in [H]}$ to denote the collection of the transition matrices, so that $\mathbb{T}_h(\cdot\given s, {a})\in\Delta({\mathcal{S}})$ gives the probability of the next state if joint action ${a}$ is taken at state $s$ and step $h$. In the following discussions, for any given $a$, we treat $\TT_h(a)\in\RR^{|\cS|\times|\cS|}$ as a matrix, where each row gives the probability for the next state. We use $\mu_1$ to denote the distribution of the initial state $s_1$, and $\cO$ {to} denote the observation space  with $|\mathcal{O}|=O$. We use $\mathbb{O}=\{\mathbb{O}_h\}_{h\in [H + 1]}$ to denote the collection of the joint emission matrices, so that $\mathbb{O}_h(\cdot\given s)\in\Delta({\mathcal{O}})$ gives the emission distribution over the joint observation space $\mathcal{O}$ at state $s$ and step $h$. For notational convenience, we will at times adopt the matrix convention, where $\OO_h$ is a matrix with rows $\OO_h(\cdot\given s_h)$. Finally, $r=\{r_{h}\}_{h\in [H]}$ is a collection of reward functions, so that $r_{h}(s_h, a_h)$ is the reward given the state $s_h$ and action $a_h$ at step $h$. We denote the trajectory with states as $\overline{\tau}_h = (s_{1:h}, o_{1:h}, a_{1:h-1})$ and the trajectory without states as $\tau_h=(o_{1:h}, a_{1:h-1})$.

\paragraph{Belief and approximate belief.} Although in a POMDP, the agent cannot see the underlying state directly, it can still form the \emph{belief} over the latent state by the historical observations and action. \begin{definition}[Belief state update]
For each $h\in [H+1]$, the Bayes operator (with respect to the joint observation)  $B_{h}:\Delta(\cS)\times \cO\rightarrow \Delta(\cS)$ is defined for $b\in\Delta(\cS)$, and $o\in\cO$ by:
\begin{align*}
    B_h(b ; o)(x)=\frac{\mathbb{O}_h(o \given x) b(x)}{\sum_{z \in \mathcal{S}} \mathbb{O}_h(o \given z) b(z)}.
\end{align*}
For each $h\in [H]$, the belief update operator $U_h: \Delta(\mathcal{S}) \times \mathcal{A} \times \mathcal{O} \rightarrow \Delta(\mathcal{S})$, is defined by 
\begin{align*}
    U_h(b ; a, o)=B_{h+1}\left(\mathbb{T}_h(a) \cdot b ; o\right),
\end{align*}
where $\mathbb{T}_h(a) \cdot b$ represents the matrix multiplication. We use the notation $b_h$ to denote the belief update function, which receives a sequence of actions and observations and outputs a distribution over states at the step $h$: the belief state at step $h=1$ is defined as $\bb_1(\emptyset) = \mu_1$. 
For any $2\le h\le H$ and any action-observation sequence $(a_{1:h-1}, o_{1:h})$, we inductively define the belief state:
\begin{align*}
    \bb_{h+1}(a_{1:h}, o_{1:h}) &= \mathbb{T}_h(a_h)\cdot \bb_{h}( a_{1:h-1}, o_{1:h}),\\
    \bb_{h}(a_{1:h-1}, o_{1:h}) &= B_{h}(\bb_{h}(a_{1:h-1}, o_{1:h-1}); o_h).
\end{align*}
We also define the approximate belief update using the most recent $L$-step history. For $1\le h \le H$, we follow the notation of \cite{golowich2022planning} and define
\begin{align*}
    \bb_h^{\mathrm{apx},\cG}(\emptyset;{D})= \begin{cases}\mu_1 & \text { if } h=1 \\ {D} & \text { otherwise },\end{cases}
\end{align*}
where ${D}\in\Delta(\cS)$ is the prior for the approximate belief update. Then for any $1\le h-L< h\le H$ and any action-observation sequence $(a_{h-L:h-1}, o_{h-L+1:h})$, we inductively define
\begin{align*}
\bb_{h+1}^{\mathrm{apx}, \cG}(a_{h-L:h}, o_{h-L+1:h};{D}) &= \mathbb{T}_h(a_h)\cdot \bb^{\mathrm{apx}, \cG}_{h}(a_{h-L:h-1}, o_{h-L+1:h};{D}),\\
\bb_{h}^{\mathrm{apx}, \cG}(a_{h-L:h-1}, o_{h-L+1:h};{D}) &= B_{h}(\bb^{\mathrm{apx}, \cG}_{h}(a_{h-L:h-1}, o_{h-L+1:h-1};{D}); o_h).
\end{align*}
For the remainder of our paper, we shall use the important initialization for the approximate belief, which are defined as $\bb^{\prime}_{h}(\cdot):=\bb_{h}^{\mathrm{apx}, \cG}(\cdot;\operatorname{Unif}(\cS))$.

\end{definition} 



\paragraph{Policy and value function.} We define a stochastic policy at step $h$ as: 
\#\label{policy}
    {\pi}_{h}: \cO^{h}\times\cA^{h-1}\rightarrow \Delta({\mathcal{A}}),
\#
where the agent necessarily requires entire history information for optimal decision making. The corresponding policy class is denoted as $\Pi_h$. We further denote $\Pi = \times_{h\in [H]} \Pi_{h}$. Meanwhile, we also consider policies that can depend on the state as $\pi_h:\cS\rightarrow\Delta(\cA)$ defined in the same way as standard Markovian policies in MDP. We denote the corresponding policy class as $\Pi_\cS:=\{\pi_{1:H}\given \pi_h:\cS\rightarrow\Delta(\cA) \text{ for any }h\in[H]\}$. Finally, we define $\Pi^{gen}:=\{\pi_{1:H}\given {\pi}_{h}: \cS^h\times\cO^{h}\times\cA^{h-1}\rightarrow \Delta({\mathcal{A}})\}$ to be the most general policy space that can potentially depend on all historical states, observations, and actions. It is easy to see that $\Pi, \Pi_\cS\in\Pi^{gen}$. 

Given the POMDP model $\cP$, we define the value function as $V_h^{\pi, \cP}(y_h):=\EE_{\pi}^{\cP}[\sum_{t=h}^H r_t(s_t, a_t)\given y_h]$, indicating the expected accumulated rewards from step $h$, where $y_h\subseteq (s_{1:h}, o_{1:h}, a_{1:h-1})$ is the available information. For $h=1$, we adopt the simplified notation $v^{\cP}(\pi)=\EE_{\pi}^\cP[\sum_{h=1}^H r_h(s_h, a_h)]$. Meanwhile, we also define $Q_h^{\pi, \cP}(y_h, a_h):=\EE_{\pi}^{\cP}[\sum_{t=h}^H r_t(s_t, a_t)\given y_h, a_h]$. We denote $d_h^{\pi, \cP}(s_h) = \PP_h^{\pi, \cP}(s_h)$ to be the occupancy on the state space. For models beyond $\cP$ like $\hat{\cM}$, we also define $V_h^{\pi, \cP}$, $Q_{h}^{\pi, \cP}$, $v^{\hat{\cM}}(\pi)$, and $d_h^{\pi, \hat{\cM}}$ accordingly. The goal of learning in POMDP is to find the optimal policy that maximizes the accumulated reward. Formally, we define
\begin{definition}[$\epsilon$-optimal policy]
	Given $\epsilon>0$, a policy $\pi^\star\in\Pi$ is $\epsilon$-optimal, if $v^{\cP}(\pi^\star)\ge \max_{\pi\in\Pi}v^\cP(\pi)-\epsilon$.
\end{definition}
\paragraph{Learning with asymmetric information.} Common RL algorithm in POMDP deals with the setting that during both training and test time, the agent can only observe its historical observations and actions, while the states are not available. In other word, the agent can only utilize policies from $\Pi$ to interact with the environment. In contrast, we deal with the scenario that during training, the agent is allowed to observe the underlying state, thus it can utilize policies from $\Pi_{gen}$ to facilitate the training. Meanwhile, the goal is still to find the optimal policy in the space of $\Pi$ since at test time, the agent cannot observe the state information anymore. 
\subsection{Model-based learning with reward-free exploration}\label{sec:reward-free}
\begin{algorithm}[!h]
\begin{algorithmic}
\caption{Reward-free exploration\label{alg:reward-free-pomdp}}

\State  \textbf{Input:} $\cP=(H, \cS, \cA, \cO, \{\TT_{h}\}_{h\in[H]}, \{\OO_h\}_{h\in[H]}, \mu_1, \{r_{h}\}_{h\in[H]})$
\For{$h\in[H], s_h\in\cS$}
	\State $\hat{r}_{h^\prime}(s_h^\prime, a_h^\prime)\leftarrow \mathbbm{1}[h^\prime=h, s_h^\prime=s_h]$ for any $h^\prime, s_h^\prime, a_h^\prime\in[H]\times\cS\times\cA$.
	\State $\Psi(h, s_h)\leftarrow\text{MDP\_Learning}(\cP, \hat{r})$
	\For{$a_h\in\cA$}
		\State Collect $N$ trajectories by executing policy $\Psi(h, s_h)$ for first $h-1$ steps then take action $a_h$ deterministically and denote the dataset $\{(s_h^i, o_{h}^i, s_{h+1}^i)\}_{i\in[N]}$.
		\State $N_{h}(s_h)\leftarrow \sum_{i\in[N]}\mathbbm{1}[s_h^i=s_h]$
		\State $N_{h}(s_h, s_{h+1})\leftarrow \sum_{i\in[N]}\mathbbm{1}[s_h^i=s_h, s_{h+1}^i=s_{h+1}]$ for any $s_{h+1}\in\cS$
		\State $N_{h}(s_h, o_{h})\leftarrow \sum_{i\in[N]}\mathbbm{1}[s_h^i=s_h, o_h^i=o_h]$ for any $o_{h}\in\cO$
		\State $\hat{\TT}_h(s_{h+1}\given s_h, a_h)\leftarrow \frac{N_{h}(s_h, s_{h+1})}{N_{h}(s_h)}$ for any $s_{h+1}\in\cS$
		\State $\hat{\OO}_h(o_h\given s_h)\leftarrow \frac{N_h(s_h, o_h)}{N_h(s_h)}$ for any $o_{h}\in\cO$
	\EndFor
\EndFor
\State Define $\hat{\cP}:=(H, \cS, \cA, \cO, \{\hat{\TT}_{h}\}_{h\in[H]}, \{\hat{\OO}_h\}_{h\in[H]}, \mu_1, \{r_{h}\}_{h\in[H]})$
\State \Return $\hat{\cP}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[!h]
\begin{algorithmic}
\caption{Learning POMDP\label{alg:optimal-plan}}
\State  \textbf{Input:} $\cP, L$
\State $\hat{\cP}\leftarrow \text{Reward\_free}(\cP)$
\State $\{\hat{\bb}^\prime_h\}_{h\in[H]}\leftarrow \text{Construct\_Belief}(\cP, L)$
\State Define the MDP $\hat{\cM}$ using $\hat{\cP}$ and $\{\hat{\bb}^\prime_h\}_{h\in[H]}$ as in \S\ref{sec:reward-free}
\State $\hat{\pi}\leftarrow\text{MDP\_Planning}(\hat{\cM})$
\State \Return $\hat{\pi}$
\end{algorithmic}
\end{algorithm}


Although a similar setting to learning with asymmetric information is studied by \cite{lee2023learning}, showing sample-efficient RL is possible with so-called \emph{hindsight observability}, their algorithm still relies on a planning oracle in POMDPs. Indeed, we remark that their algorithm cannot be computationally tractable since the assumption of hindsight observability only changes the interaction protocol with the environment, and its computational complexity cannot be better than planning in POMDP, which a is \texttt{PSAPCE-complete} problem \citep{papadimitriou1987complexity}. Therefore, to circumvent such hardness, we make the following standard assumption that has enabled quasi-polynomial time planning algorithms in solving POMDPs \citep{golowich2022planning,golowich2022learning}.

\begin{assumption}[$\gamma$-observability]\label{assump:observa}
	Let $\gamma> 0$. For $h\in [H]$, we say that the matrix $\OO_h$ satisfies the $\gamma$-observability assumption if for each $h\in[H]$, for any $b, b^\prime\in \Delta(\cS)$,
\begin{align*}
\left\|\mathbb{O}_{h}^{\top} b-\mathbb{O}_{h}^{\top} b^{\prime}\right\|_{1} \geq \gamma\left\|b-b^{\prime}\right\|_{1}.
\end{align*}
A POMDP satisfies (one-step) $\gamma$-observability if all its $\OO_h$ for  $h\in[H]$ do so.  

Now with Assumption \ref{assump:observa}, our algorithm will first explore the POMDP in a reward-free manner with the help of asymmetric information to learn an approximate POMDP $\hat{\cP}$ and an approximate belief function $\hat{\bb}_{1:H}^\prime$. After the exploration stage, we will solve a planning problem for an MDP $\hat{\cM}$ which has the state space $\cZ_h:=(\cA\times\cO)^{\min\{L, h\}}$ for each $h\in[H]$ and action space the same as $\cA$. More importantly, we define the transition of $\hat{\cM}$ as 
\$
\PP_{h}^{\hat{\cM}}(z_{h+1}\given z_h, a_h)&:=\sum_{s_{h}, s_{h+1}}\hat{\bb}_h^\prime(z_h)(s_h)\hat{\TT}_h(s_{h+1}\given s_h, a_h)\hat{\OO}_h(o_{h+1}\given s_{h+1}),\\
r_h^{\hat{\cM}}(z_h, a_h)&:=\EE_{s_h\sim\hat{\bb}_h^\prime(z_h)}[r_{h}(s_h, a_h)].
\$
for $z_{h+1}=(o_{h-L+1:h+1}, a_{h-L+1:h})$,$z_h=(o_{h-L:h}, a_{h-L:h-1})$.
\end{assumption}
The first step is to learn an approximate POMDP model, i.e., $\hat{\TT}_{1:H}$ and $\hat{\OO}_{1:H}$, the guarantee of which is stated in the following theorem.
\begin{theorem}\label{lem:free}
	Algorithm \ref{alg:reward-free-pomdp} can learn the approximate POMDP with transition $\hat{\TT}_{1:H}$ and emission $\hat{\OO}_{1:H}$ such that for any policy $\pi\in\Pi^{gen}$ and $h\in[H]$
	\$
	\EE_{\pi}^\cP \bigg(\|\TT_{h}(\cdot\given s_h, a_h)-\hat{\TT}_{h}(\cdot\given s_h, a_h)\|_1+\|\OO_{h}(\cdot\given s_h)-\hat{\OO}_{h}(\cdot\given s_h)\|_1\bigg)\le\epsilon,
	\$
	using sample complexity $\tilde{\cO}(\frac{S^2AHO+S^3AH}{\epsilon^2}+\frac{S^4A^2H^5}{\epsilon})$ with probability $1-\delta$.
\end{theorem}
\begin{proof}
Note by Lemma \ref{lem:state} it suffices to consider only $\pi\in\Pi_\cS$ (by considering $r_{h}(s_h, a_h):=\|\TT_{h}(\cdot\given s_h, a_h)-\hat{\TT}_{h}(\cdot\given s_h, a_h)\|_1+\|\OO_{h}(\cdot\given s_h)-\hat{\OO}_{h}(\cdot\given s_h)\|_1$). 
	For each $h\in[H]$ and $s_h\in\cS$, we define 
	\$
	p_h(s_h) = \max_{\pi\in\Pi_\cS}d_h^{\pi}(s_h).
	\$
	Fix $\epsilon_1> 0$, we define $\cU(h, \epsilon_1) = \{s_h\in\cS\given p_h(s_h)\ge \epsilon_1\}$. By \cite{jin2020reward}, one can learn the policy $\Psi(h, s_h)$ with sample complexity $\tilde{\cO}(\frac{S^2AH^4}{\epsilon_1})$ such that $d_h^{\Psi(h, s_h)}(s_h)\ge \frac{p_h(s_h)}{2}$ for each $s_h\in\cU(h, \epsilon_1)$ with probability $1-\delta_1$. Now we assume this event holds for any $h\in[H]$ and $s_h\in\cU(h, \epsilon_1)$. For each $s_h\in\cS$ and $a_h\in\cA$, we have executed the policy $\Psi(h, s_h)$ followed by an action $a_h\in\cA$ for $N$ episodes and denote the number of episodes that $s_h$ and $a_h$ are visited as $N_h(s_h, a_h)$. Then with probability $1-e^{N\epsilon_1/8}$, $N_h(s_h, a_h)\ge \frac{Np_h(s_h)}{2}$ by chernoff bound.
	Now conditioned on this event, we are ready to evaluate the following
	\$
	\EE_{\pi}^\cP \|\TT_{h}(\cdot\given s_h, a_h)-\hat{\TT}_{h}(\cdot\given s_h, a_h)\|_1&= \sum_{s_h, a_h}d_h^\pi(s_h)\pi_h(a_h\given s_h) \|\TT_{h}(\cdot\given s_h, a_h)-\hat{\TT}_{h}(\cdot\given s_h, a_h)\|_1\\
	&\le S\epsilon_1 + \sum_{s_h\in\cU(h, \epsilon_1), a_h}d_h^\pi(s_h)\pi_h(a_h\given s_h) \sqrt{\frac{2S\log(1/\delta_2)}{Np_h(s_h)}}\\
	&\le S\epsilon_1 + \sum_{s_h} \sqrt{d^\pi_h(s_h)}\sqrt{\frac{S\log(1/\delta_2)}{N}}\\
	&=S\epsilon_1 + S\sqrt{\frac{\log(1/\delta_2)}{N}}.
	\$
	Similarly, 
	\$
	\EE_{\pi}^\cP \|\OO_{h}(\cdot\given s_h)-\hat{\OO}_{h}(\cdot\given s_h)\|_1
	&=\sum_{s_h}d_h^\pi(s_h)\|\OO_{h}(\cdot\given s_h)-\hat{\OO}_{h}(\cdot\given s_h)\|_1\\
	&\le S\epsilon_1 + \sum_{s_h\in\cU(h, \epsilon_1)}d_h^\pi(s_h)\sqrt{\frac{O\log(1/\delta_2)}{Np_h(s_h)}}\\
	&\le S\epsilon_1 + \sum_{s_h\in\cU(h, \epsilon_1)}\sqrt{d_h^\pi(s_h)}\sqrt{\frac{O\log(1/\delta_2)}{N}}\\
	&\le S\epsilon_1 + \sqrt{\frac{SO\log(1/\delta_2)}{N}}.
	\$
	Therefore, by a union bound, the all high probability events hold with probability 
	\$
	1-SH\delta_1-SHAe^{N\epsilon_1/8}-SAH\delta_2.
	\$
	Therefore, we can choose $N=\tilde{\cO}(\frac{S^2+SO}{\epsilon^2})$ and $\epsilon_1=\cO(\frac{\epsilon}{S})$, leading to the total sample complexity 
	\$
	SHA(N+\tilde{\cO}(\frac{S^3AH^4}{\epsilon})) = \tilde{\cO}(\frac{S^2AHO+S^3AH}{\epsilon^2}+\frac{S^4A^2H^5}{\epsilon})
	\$
\end{proof}

With the guarantee of the learned $\hat{\TT}_{1:H}$ and $\hat{\OO}_{1:H}$, we show that the approximately  optimal policy of $\hat{\cM}$ is also an approximately optimal policy of $\cP$.
\begin{theorem}\label{lem:error}
	For $\hat{\cP}$ of Algorithm \ref{alg:reward-free-pomdp}, we define its approximate belief $\hat{\bb}^\prime_{1:H}$ similarly for $\cP$ and 
	\$
	\epsilon_{model}:&=\max_{\pi\in\Pi_L}\EE_{\pi}^\cP\sum_{h}\|\TT_{h}(\cdot\given s_h, a_h)-\hat{\TT}_{h}(\cdot\given s_h, a_h)\|_1+\|\OO_{h}(\cdot\given s_h)-\hat{\OO}_{h}(\cdot\given s_h)\|_1\\
	\epsilon_{belief}:&=\max_{\pi\in\Pi_L, h\in[H]}\EE_{\pi}^\cP\|\bb_h(\tau_h)-\hat{\bb}_h^\prime(z_h)\|_1.
	\$
	Denote $\pi^\star\in\arg\max_{\pi\in\Pi_L} v^{\cP}(\pi)$.
	It holds that 
	\$
	v^{\cP}(\pi^\star)\le v^{\cP}(\hat{\pi}) + 2(H\epsilon_{model}+H^2\epsilon_{belief}).
	\$
\end{theorem}	
\begin{proof}
	Note that
	\$
	&\EE_{\pi^\star}^\cP [V_{h}^{\pi^\star, \cP}(\tau_h)-V_{h}^{\hat{\pi}, \hat{\cM}}(z_h)]\le \EE_{\pi^\star}^\cP [Q_{h}^{\pi^\star, \cP}(\tau_h, a_{h}^\star)-Q_{h}^{\hat{\pi}, \hat{\cM}}(z_h, a_h^\star)]\\
	&\le \EE_{\pi^\star}^\cP [\EE_{s_{h}\sim b_{h}(\tau_h), a_h^\star\sim\pi_{h}^\star(\cdot\given z_h), s_{h+1}\sim \TT_{h}(\cdot\given s_h, a_h^\star), o_{h+1}\sim\OO_{h+1}(\cdot\given s_{h+1})}[r_{h}(s_h, a^\star_h) + V_{h+1}^{\pi^\star, \cP}(\tau_{h+1})]\\
	&\quad-\EE_{s_{h}\sim \hat{b}_{h}^\prime(z_h), a_h^\star\sim\pi_{h}^\star(\cdot\given z_h), s_{h+1}\sim \hat{\TT}_{h}(\cdot\given s_h, a_h^\star), o_{h+1}\sim\hat{\OO}_{h+1}(\cdot\given s_{h+1})}[r_{h}(s_h, a^\star_h)+V_{h+1}^{\hat{\pi}, \hat{\cM}}(z_{h+1})]]\\
	&\le \EE_{\pi^\star}^\cP [(H-h)\sum_{s_h, a_h^\star, s_{h+1}, o_{h+1}}|\pi_{h}^\star(a_h^\star\given z_h)b_h(\tau_h)(s_h)\TT_{h}(s_{h+1}\given s_h, a_h^\star)\OO_{h+1}(o_{h+1}\given s_{h+1})-\pi_{h}^\star(a_h^\star\given z_h)\hat{b}_h^\prime(z_h)(s_h)\hat{\TT}_{h}(s_{h+1}\given s_h, a_h^\star)\hat{\OO}_{h+1}(o_{h+1}\given s_{h+1})| \\
	&\quad+\EE_{s_{h}\sim b_{h}(\tau_h), a_h^\star\sim\pi_{h}^\star(\cdot\given z_h), s_{h+1}\sim \TT_{h}(\cdot\given s_h, a_h^\star), o_{h+1}\sim\OO_{h+1}(\cdot\given s_{h+1})}[V_{h+1}^{\pi^\star, \cP}(\tau_{h+1})-V_{h+1}^{\hat{\pi}, \hat{\cM}}(z_{h+1})]]\\
	&\le (H-h)\EE_{\pi^\star}^\cP [\|b_h(\tau_h)-\hat{b}_h^\prime(z_h)\|_1 + \|\TT_{h}(\cdot\given s_h, a_{h})-\hat{\TT}_{h}(\cdot\given s_h, a_{h})\|_1+ \|\OO_{h+1}(\cdot\given s_{h+1})-\hat{\OO}_{h+1}(\cdot\given s_{h+1})\|_1] \\
	&\quad+\EE_{\pi^\star}^\cP[V_{h+1}^{\pi^\star, \cP}(\tau_{h+1})-V_{h+1}^{\hat{\pi}, \hat{\cM}}(z_{h+1})].
	\$ 
	Therefore, by telescoping from $h=1$ to $H$, we conclude that
	\$
	v^{\cP}(\pi^\star)-v^{\hat{\cM}}(\hat{\pi})\le H\epsilon_{model}+H^2\epsilon_{belief}.
	\$
	Similarly, we consider 
	\$
	&\EE_{\hat{\pi}}^\cP [V_{h}^{\hat{\pi}, \hat{\cM}}(z_h)-V_{h}^{\hat{\pi}, \cP}(\tau_h)]= \EE_{\hat{\pi}}^\cP[Q_{h}^{\hat{\pi}, \hat{\cM}}(z_h, \hat{a}_{h})-Q_{h}^{\hat{\pi}, \cP}(\tau_h, \hat{a}_{h})]\\
	&\le \EE_{\hat{\pi}}^\cP [\EE_{s_{h}\sim \hat{b}_{h}^\prime(z_h), \hat{a}_h\sim\hat{\pi}_h(\cdot\given z_h), s_{h+1}\sim \hat{\TT}_{h}(\cdot\given s_h, \hat{a}_h), o_{h+1}\sim\hat{\OO}_{h+1}(\cdot\given s_{h+1})}[r_{h}(s_h, \hat{a}_h)+V_{h+1}^{\hat{\pi}, \hat{\cM}}(z_{h+1})]\\
	&\quad-\EE_{s_{h}\sim b_{h}(\tau_h), \hat{a}_h\sim\hat{\pi}_h(\cdot\given z_h), s_{h+1}\sim \TT_{h}(\cdot\given s_h, \hat{a}_h), o_{h+1}\sim\OO_{h+1}(\cdot\given s_{h+1})}[r_{h}(s_h, \hat{a}_h) + V_{h+1}^{\pi^\star, \cP}(\tau_{h+1})]]\\
	&\le \EE_{\hat{\pi}}^\cP [(H-h)\sum_{s_h, \hat{a}_h, s_{h+1}, o_{h+1}}|\hat{\pi}_h(\hat{a}_h\given z_h),b_h(\tau_h)(s_h)\TT_{h}(s_{h+1}\given s_h, \hat{a}_h)\OO_{h+1}(o_{h+1}\given s_{h+1})-\hat{\pi}_h(\hat{a}_h\given z_h)\hat{b}_h^\prime(z_h)(s_h)\hat{\TT}_{h}(s_{h+1}\given s_h, \hat{a}_h)\hat{\OO}_{h+1}(o_{h+1}\given s_{h+1})| \\
	&\quad+\EE_{s_{h}\sim b_{h}(\tau_h), s_{h+1}\sim \TT_{h}(\cdot\given s_h, \hat{a}_h), o_{h+1}\sim\OO_{h+1}(\cdot\given s_{h+1})}[V_{h+1}^{\hat{\pi}, \hat{\cM}}(z_{h+1})-V_{h+1}^{\hat{\pi}, \cP}(\tau_{h+1})]]\\
	&\le (H-h)\EE_{\hat{\pi}}^\cP [\|b_h(\tau_h)-\hat{b}_h^\prime(z_h)\|_1 + \|\TT_{h}(\cdot\given s_h, a_{h})-\hat{\TT}_{h}(\cdot\given s_h, a_{h})\|_1+ \|\OO_{h+1}(\cdot\given s_{h+1})-\hat{\OO}_{h+1}(\cdot\given s_{h+1})\|_1] \\
	&\quad+\EE_{\hat{\pi}}^\cP[V_{h+1}^{\hat{\pi}, \hat{\cM}}(z_{h+1})-V_{h+1}^{\hat{\pi}, \cP}(\tau_{h+1})].
	\$
	Therefore, by telescoping from $h=1$ to $H$, we conclude that
	\$
	v^{\hat{\cM}}(\hat{\pi})-v^{\cP}(\hat{\pi})\le H\epsilon_{model}+H^2\epsilon_{belief}.
	\$
	Finally, we have
	\$
	v^{\cP}(\pi^\star)-v^{\cP}(\hat{\pi})\le v^{\cP}(\pi^\star)-v^{\hat{\cM}}(\hat{\pi})+ v^{\hat{\cM}}(\hat{\pi})-v^{\cP}(\hat{\pi}) \le 2(H\epsilon_{model}+H^2\epsilon_{belief}).
	\$
\end{proof}
Now combing Theorem \ref{lem:free} and \ref{lem:error}, we are finally ready to state the sample and computation complexity guarantee of Algorithm \ref{alg:reward-free-pomdp}
\begin{theorem}\label{thm:pomdp-main}
	Fix $\epsilon, \delta>0$. Under Assumption \ref{assump:observa}, Algorithm \ref{alg:optimal-plan} can learn an $\epsilon$-optimal policy of $\cP$ with probability $1-\delta$ with sample complexity $\tilde{\cO}(\frac{S^2AHO+S^3AH}{\epsilon^2}+\frac{S^4A^2H^5}{\epsilon})$ and computation complexity $H(OA)^{\cO(\log(SH/\epsilon)/\gamma^4)}$
\end{theorem}
\begin{proof}
	By combing Theorem \ref{lem:free} and \ref{lem:error}, it is guaranteed that Algorithm \ref{alg:reward-free-pomdp} can learn an $\epsilon$-optimal policy of $\cP$ in the policy class $\Pi_L$. Then by choosing $L=\cO(\log(SH/\epsilon)/\gamma^4)$, according to \cite{golowich2022planning}, an $\epsilon$-optimal policy in the policy class $\Pi_L$ is also an $\cO(\epsilon)$-optimal in the policy class $\Pi$, proving the theorem.
\end{proof}

\subsection{Supporting technical details}
In the following, we provide the some technical lemmas and the proof.

\begin{lemma}\label{lem:trick}
	Fix two sets $\cX$, $\cY$ and two joint distributions $P_1, P_2\in\Delta(\cX\times\cY)$. It holds that
	\$
	 - \EE_{P_1(x)}\sum_y|P_{1}(y\given x)-P_{2}(y\given x)|\le \sum_{x, y}|P_1(x, y)-P_2(x, y)|-\sum_x|P_1(x)-P_2(x)|\le \EE_{P_1(x)}\sum_y|P_{1}(y\given x)-P_{2}(y\given x)|
	\$
\end{lemma}

\begin{proof}
For the second inequality, it holds that
	\$
	\sum_{x, y}|P_1(x, y)-P_2(x, y)|&=\sum_{x, y}|P_1(x, y)-P_1(x)P_2(y\given x)+P_1(x)P_2(y\given x)-P_2(x, y)|\\
	&\le \sum_{x, y}|P_1(x, y)-P_1(x)P_2(y\given x)|+|P_1(x)P_2(y\given x)-P_2(x, y)|\\
	&= \sum_{x, y}|P_1(x)(P_1(y\given x)-P_2(y\given x))|+|P_2(y\given x)(P_1(x)-P_2(x))|\\
	&= \EE_{P_1(x)}\sum_y|P_{1}(y\given x)-P_{2}(y\given x)|+\sum_x|P_1(x)-P_2(x)|.
	\$
	Meanwhile, for the first inequality, it holds that

		\$
	\sum_{x, y}|P_1(x, y)-P_2(x, y)|&=\sum_{x, y}|P_1(x, y)-P_1(x)P_2(y\given x)+P_1(x)P_2(y\given x)-P_2(x, y)|\\
	&\ge -\sum_{x, y}|P_1(x, y)-P_1(x)P_2(y\given x)|+|P_1(x)P_2(y\given x)-P_2(x, y)|\\
	&= -\sum_{x, y}|P_1(x)(P_1(y\given x)-P_2(y\given x))|+|P_2(y\given x)(P_1(x)-P_2(x))|\\
	&= -\EE_{P_1(x)}\sum_y|P_{1}(y\given x)-P_{2}(y\given x)|+\sum_x|P_1(x)-P_2(x)|,
	\$
concluding our lemma.
\end{proof}
\begin{lemma}\label{lem:traj}
	Consider any two POMDP instances $\cP$ and $\hat{\cP}$ and define the belief functions as $\bb_{1:H}$ and $\hat{\bb}_{1:H}$,  respectively. It holds that for any $\pi$
	\$
	\sum_{\overline{\tau}_H}|\PP^{\pi, \cP}(\overline{\tau}_H)-\PP^{\pi, \hat{\cP}}(\overline{\tau}_H)|\le \EE_{\pi}^\cP\sum_{h\in[H]}\|\TT_{h}(\cdot\given s_h, a_h)-\hat{\TT}_{h}(\cdot\given s_h, a_h)\|_1+\|\OO_{h}(\cdot\given s_h)-\hat{\OO}_{h}(\cdot\given s_h)\|_1. 
	\$
	
	\$
		\EE_{\pi}^\cP\|b_H(\tau_H)-\hat{b}_H(\tau_H)\|_1\le 2\EE_{\pi}^\cP\sum_{h\in[H]}\|\TT_{h}(\cdot\given s_h, a_h)-\hat{\TT}_{h}(\cdot\given s_h, a_h)\|_1+\|\OO_{h}(\cdot\given s_h)-\hat{\OO}_{h}(\cdot\given s_h)\|_1.
	\$
\end{lemma}
\begin{proof}
	The first inequality also appears in \cite{lee2023learning} and we provide a simplified proof here for completeness. By Lemma \ref{lem:trick}, it holds that
	\$
		&\sum_{\overline{\tau}_H}|\PP^{\pi, \cP}(\overline{\tau}_H)-\PP^{\pi, \hat{\cP}}(\overline{\tau}_H)|\le \sum_{\overline{\tau}_{H-1}}|\PP^{\pi, \cP}(\overline{\tau}_{H-1})-\PP^{\pi, \hat{\cP}}(\overline{\tau}_{H-1})| \\
		&+ \EE_{\pi}^\cP\sum_{a_{H-1}, s_{H}, o_{H}}|\pi_{H-1}(a_{h-1}\given \overline{\tau}_{H-1})\TT_{H-1}(s_H\given s_{H-1}, a_{H-1})\OO_{H}(o_H\given s_H)-\pi_{H-1}(a_{h-1}\given \overline{\tau}_{H-1})\hat{\TT}_{H-1}(s_H\given s_{H-1}, a_{H-1})\hat{\OO}_{H}(o_H\given s_H)|\\
		&\le \sum_{\overline{\tau}_{H-1}}|\PP^{\pi, \cP}(\overline{\tau}_{H-1})-\PP^{\pi, \hat{\cP}}(\overline{\tau}_{H-1})|+ \EE_{\pi}^\cP\|\TT_{H-1}(\cdot\given s_{H-1}, a_{H-1})-\hat{\TT}_{H-1}(\cdot\given s_{H-1}, a_{H-1})\|_1+\|\OO_{H}(\cdot\given s_{H})-\hat{\OO}_{H}(\cdot\given s_H)\|_1,
	\$
	where the last step is again from Lemma \ref{lem:trick}. Therefore, by rolling out the inequality repeatedly, we proved the first result.
	
	For the second result, we notice that by Lemma \ref{lem:trick}, it holds that
	\$
	\sum_{\tau_h, s_h}|\PP_h^{\pi, \cP}(\tau_h, s_h)-\PP_h^{\pi, \hat{\cP}}(\tau_h, s_h)|\ge -\sum_{\tau_h}|\PP_h^{\pi, \cP}(\tau_h)-\PP_h^{\pi, \hat{\cP}}(\tau_h)|+\EE_{\pi}^{\cP}\sum_{s_h}|\PP_h^{\pi, \cP}(s_h\given \tau_h)-\PP_h^{\pi, \hat{\cP}}(s_h\given \tau_h)|.
	\$
	Notice the fact that $\PP_h^{\pi, \cP}(s_h\given \tau_h)$ does not depend on $\pi$ since it is exactly $\bb_h(\tau_h)(s_h)$, we conclude that
	\$
	\EE_{\pi}^{\cP}\|\bb_h(\tau_h)-\hat{\bb}_h(\tau_h)\|_1\le \sum_{\tau_h, s_h}|\PP_h^{\pi, \cP}(\tau_h, s_h)-\PP_h^{\pi, \hat{\cP}}(\tau_h, s_h)|+\sum_{\tau_h}|\PP_h^{\pi, \cP}(\tau_h)-\PP_h^{\pi, \hat{\cP}}(\tau_h)|\le 2\sum_{\overline{\tau}_H}|\PP^{\pi, \cP}(\overline{\tau}_h)-\PP^{\pi, \hat{\cP}}(\overline{\tau}_h)|,
	\$
	where the last step comes from the fact that after marginalization, the total variation distance will not increase. By combining it with the first result, we proved the second result. 
\end{proof}
\begin{lemma}\label{lem:belief}
	Consider any two POMDP instances $\cP$ and $\hat{\cP}$ and define the approximate belief functions as $\bb^\prime_{1:H}$ and $\hat{\bb}^\prime_{1:H}$ respectively. It holds that for any $\pi$ and $h\in[H]$
	\$
	\EE_{\pi}^{\cP}\|\bb_{h}(\tau_h)-\hat{\bb}^{\prime, \trunc}_{h}(z_h)\|_1\le \epsilon. 
	\$
\end{lemma}

\begin{proof}
	We firstly evaluate the observability of an estimated emission $\hat{\OO}_h$ as follows
	\$
	\|\hat{\OO}_h^\top (b-b^\prime)\|_1\ge \|\OO_h^\top (b-b^\prime)\|_1-\|(\OO_h^\top-\hat{\OO}_h^\top) (b-b^\prime)\|_1\ge (\gamma-\|\hat{\OO}_h-\OO_h\|_{\infty})\|b-b^\prime\|_1,
	\$
	for any $b, b^\prime\in\Delta(\cS)$ and $\|\hat{\OO}_h-\OO_h\|_{\infty}:=\max_{s_h\in\cS}\|\OO_h(\cdot\given s_h)-\hat{\OO}_h(\cdot\given s_h)\|_1$. Therefore, if one can ensure that the emission at any state $s_h$ is learned accurately in the sense that $\|\OO_h(\cdot\given s_h)-\hat{\OO}_h(\cdot\given s_h)\|_1\le \frac{\gamma}{2}$, we can conclude that $\hat{\OO}_h$ is also $\gamma/2$-observable. However, the key challenge here is that there could exist some states $s_h$ at level $h$ that can only be visited with a low probability no matter what exploration policy is used. Therefore, emission at such states may not be learned accurately. 
	
	To circumvent this issue, our key technique here is to \emph{redirect} the transition probability into states that cannot be explored sufficiently to a new state $s^{\text{exit}}$, the emission associated with which gives a new observation $o^{\text{exit}}$ deterministically. Formally, for $\epsilon_1>0$, we define 
	\$
	\cS^{\text{low}}_h:=\{s_h\in\cS\given \frac{N_h(s_h)}{N}< \frac{\epsilon_1}{2}\}, \quad \cS^{\text{high}}_h:=\cS\setminus \cS^{\text{low}}_h
	\$
	With Chernoff bound, with probability at least $1-Se^{-N\epsilon_1/8}$, it holds that
	\$
	\cS^{\text{low}}_h\subseteq \{s_h\in\cS\given p_{h}(s_h))< \epsilon_1\}.
	\$
	To see the reason, we notice that for any $s_h$ such that $p_{h}(s_h)\ge \epsilon_1$, with probability $1-e^{-N\epsilon_1/8}$, it holds that $\frac{N_h(s_h)}{N}\ge \frac{\epsilon_1}{2}$. Therefore, the last step is by taking a union bound for all $s_h$. Now with $\cS^{\text{low}}_h$ defined, we are ready to construct a truncated pomdp $\cP^{\text{trunc}}$ such that for each $h\in[H]$, we define its non-stationary state space as 
	\$
	\cS_h^{\text{trunc}}:=\cS^{\text{high}}_h\cup\{s^{\text{exit}}\}.
	\$
	Meanwhile, we also extend the observation space as
	\$
	\cO_h^{\text{trunc}}:=\cO\cup\{o^{\text{exit}}\}.
	\$
	For transition, we define
	\$
	\TT_h^{\text{trunc}}(s_{h+1}\given s_h, a_h) = \TT_{h}(s_{h+1}\given s_h, a_h), \forall s_h, s_{h+1}\in\cS_{h+1}^{\text{high}}, a_h\in \cA.
	\$
	Meanwhile, we define
	\$
	\TT_{h}^{\text{trunc}}(s^{\text{exit}}\given s_h, a_h)=1-\sum_{s_{h+1}\in\cS_{h+1}^{\text{low}}}\TT_h(s_{h+1}\given s_h, a_h), \forall s_h\in\cS_{h+1}^{\text{high}}.
	\$
	Once the state becomes $s^{\text{exit}}$, future states will always be $s^{\text{exit}}$ no matter what actions are taken.
	For emission, we define
	\$
	\OO_{h}^{\text{trunc}}(o_h\given s_{h}):=\OO_{h}(o_h\given s_h), \forall s_h\in\cS_{h}^{\text{high}}, o_h\in\cO_h,	
	\$
	and 
	\$
	\OO_h^{\text{trunc}}(o^{\text{exit}}\given s^{\text{exit}}) = 1.
	\$
	Finally, the reward associated with $s^{\text{exit}}$ is $0$ for any actions. Now we examine the total variation distance of trajectory distribution in $\cP$ and $\cP^\trunc$.
	For any policy $\pi\in\Pi^{\text{gen}}$, it is easy to see that
	\$
	\PP^{\pi, \cP}(\overline{\tau}_H)=\PP^{\pi, \cP^\trunc}(\overline{\tau}_H),
	\$
	for any $\overline{\tau}_H\in\overline{\cT}_H^{\high}:=\{(s_{1:H}, o_{1:H}, a_{1:H})\given s_{h}\in\cS_h^{\high}, \forall h\in[H]\}$. Meanwhile, it holds that
	\$
	\PP^{\pi, \cP}(\overline{\tau}_H\not\in\overline{\cT}_H^{\high})\le \sum_{h}\PP_h^{\pi, \cP}(s_h\in\cS^{\low}_h)\le HS\epsilon_1.
	\$
	Therefore, the total variation distance of trajectory distribution in $\cP$ and $\cP^\trunc$ can be bound by 
	\$
	\sum_{\overline{\tau}_H}|\PP^{\pi, \cP}(\overline{\tau}_H)-\PP^{\pi, \cP^\trunc}(\overline{\tau}_H)|\le 2HS\epsilon_1.
	\$
	On the other hand, by Lemma \ref{lem:traj}, we have
	\$
	\EE_{\pi}^{\cP}[\|\bb_h(\tau_h)-\bb_h^{\trunc}(\tau_h)\|_1]&\le \EE_{\pi}^{\cP}\sum_{t\in[h]}\|\TT_{t}(\cdot\given s_t, a_t)-\TT^\trunc_{t}(\cdot\given s_t, a_t)\|_1+\|\OO_{t}(\cdot\given s_t)-\OO^{\trunc}_{t}(\cdot\given s_t)\|_1\\
	&\le 4\PP^{\pi, \cP}(\exists t\in[h]: s_t\not\in\cS_t^\high)\\
	&\le 4HS\epsilon_1.
	\$
	Now we are ready to examine $\hat{\bb}_h^{\prime, \trunc}$. Since $\hat{\cP}^\trunc$ is $\gamma/2$-observable, by \cite{golowich2022planning}, it holds that 
	\$
	\EE^{\hat{\cP}^\trunc}_\pi\|\hat{\bb}_h^{\trunc}(\tau_h)-\hat{\bb}_h^{\prime,\trunc}(z_h)\|_1\le \epsilon_2.
	\$
	For the total variation distance of trajectory distributions between $\cP^\trunc$ and $\hat{\cP}^\trunc$, it holds that
	\$
	\sum_{\overline{\tau}_H}|\PP^{\pi, \cP^\trunc}(\overline{\tau}_H)-\PP^{\pi, \hat{\cP}^\trunc}(\overline{\tau}_H)|&\le \EE_{\pi}^{\cP^\trunc}\sum_{h}\|\TT^\trunc_{h}(\cdot\given s_h, a_h)-\hat{\TT}^\trunc_{h}(\cdot\given s_h, a_h)\|_1+\|\OO_{h}^\trunc(\cdot\given s_h)-\hat{\OO}^\trunc_{h}(\cdot\given s_h)\|_1\\
	&=\sum_{h}\EE_{\pi}^{\cP^\trunc}\mathbbm{1}[s_h\not=s^{\text{exit}}](\|\TT_{h}(\cdot\given s_h, a_h)-\hat{\TT}_{h}(\cdot\given s_h, a_h)\|_1+\|\OO_{h}(\cdot\given s_h)-\hat{\OO}_h(\cdot\given s_h)\|_1)\\
	&\le \epsilon_3,
	\$
	where the last step is due to the fact that states with non-zero visitation probability in $\cP^\trunc$ belong to $\cS_h^{\high}\cup\{s^{\text{exit}}\}$, which can be visited with sufficient probability and the corresponding transition and emission can be learned accurately. Hence, by Lemma \ref{lem:traj}, it holds that
	\$
	\EE^{\cP^\trunc}_\pi\|\bb_h^{\trunc}(\tau_h)-\hat{\bb}^\trunc_h(\tau_h)\|_1\le\epsilon_3.
	\$
	Finally, we are ready to prove
	\$
	\EE^{\cP}_\pi&\|\bb_h(\tau_h)-\hat{\bb}_h^{\prime,\trunc}(z_h)\|_1\le \EE^{\cP}_\pi\|\bb_h(\tau_h)-\bb_h^{\trunc}(\tau_h)\|_1+\EE^{\cP}_\pi\|\bb_h^{\trunc}(\tau_h)-\hat{\bb}^\trunc_h(\tau_h)\|_1+\EE^{\cP}_\pi\|\hat{\bb}^\trunc_h(\tau_h)-\hat{\bb}^{\prime, \trunc}_h(z_h)\|_1\\
	&\le \EE^{\cP}_\pi\|\bb_h(\tau_h)-\bb_h^{\trunc}(\tau_h)\|_1+\EE^{\cP^\trunc}_\pi\|\bb_h^{\trunc}(\tau_h)-\hat{\bb}^\trunc_h(\tau_h)\|_1+\EE^{\hat{\cP}^\trunc}_\pi\|\hat{\bb}^\trunc_h(\tau_h)-\hat{\bb}^{\prime, \trunc}_h(\tau_h)\|_1 \\
	&\quad\quad+ 4\|\PP^{\pi, \cP}-\PP^{\pi, \cP^\trunc}\|_1+2\|\PP^{\pi, \cP^\trunc}-\PP^{\pi, \hat{\cP}\trunc}\|\\
	&\le 4HS\epsilon_1 + \epsilon_3 +\epsilon_2 + 8HS\epsilon_1+2\epsilon_3\\
	&\le 12HS\epsilon_1+\epsilon_2+\epsilon_3.
	\$
\end{proof}

%\begin{proof}
%	Note that for $h\le L$, it is implied by Lemma \ref{lem:traj}. Now we consider case $h>L$.  
%	\$
%	\EE_{\pi}^{\cP}\|b^\prime_{h}(z_h)-\hat{b}^\prime_{h}(z_h)\|_1=\sum_{\tau_{h-L}}\PP^{\pi, \cP}(\tau_{h-L})\sum_{z_h}\PP^{\pi, \cP}(z_h\given \tau_{h-L})\|b^\prime_{h}(z_h)-\hat{b}^\prime_{h}(z_h)\|_1.
%	\$
%	Now we define $\cP^{\tau_{h-L}}$ be a truncated version of $\cP$ such that the transition $\TT_{h}^{\tau_{h-L}}$ and emission $\OO_h^{\tau_{h-L}}$ of $\cP^{\tau_{h-L}}$ satisfy that $\TT^{\tau_{h-L}}_h = \TT_{h+L}$, $\OO_{h}^{\tau_{h-L}}=\OO_{h+L}$ and the initial state $\rho^{\tau_{h-L}}=b_{h-L}(\tau_{h-L})$. Meanwhile, we define $\overline{\cP}^{\tau_{h-L}}$ to be the same as $\cP^{\tau_{h-L}}$ except the initial state distribution is $\text{Unif}(\cS)$. We use the notation $\pi^{\tau_{h-L}}$ to denote the partial function $\pi(\cdot\given \tau_{h-L}, \cdot)$. Now we have for any $\tau_{h-L}$, it holds that
%	\$
%	\sum_{z_h}\PP^{\pi, \cP}(z_h\given \tau_{h-L})&\|b^\prime_{h}(z_h)-\hat{b}^\prime_{h}(z_h)\|_1=\EE^{\cP^{\tau_{h-L}}}_{\pi^{\tau_{h-L}}}[\|b^\prime_{h}(z_h)-\hat{b}^\prime_{h}(z_h)\|_1]\\
%	&\le S\EE^{\overline{\cP}^{\tau_{h-L}}}_{\pi^{\tau_{h-L}}}[\|b^\prime_{h}(z_h)-\hat{b}^\prime_{h}(z_h)\|_1]\le S\EE^{\overline{\cP}^{\tau_{h-L}}}_{\pi^{\tau_{h-L}}}[\sum_{t=h-L}^h \|\TT_{t}(\cdot\given s_t, a_t)-\hat{\TT}_{t}(\cdot\given s_t, a_t)\|_1+\|\OO_{t}(\cdot\given s_t)-\hat{\OO}_{t}(\cdot\given s_t)\|_1]
%	\$
%\end{proof}
\begin{lemma}\label{lem:state}
	For any reward function $r_{1:H}$ of $\cP$ with $r_{h}:\cS\times\cA\rightarrow\RR$ for any $h\in[H]$, it holds that
	\$
	\max_{\pi\in\Pi^{gen}} v^{\cP}(\pi)\le  \max_{\pi\in\Pi_\cS} v^{\cP}(\pi)
	\$
\end{lemma}
\begin{proof}
	Denote $\pi^\star\in\Pi_\cS$ to be the optimal policy obtained by running value iteration only on the state space for $\cP$. Now we are ready to prove the following argument for any $\pi\in\Pi^{gen}$ inductively.
	\$
	Q_{h}^{\pi^\star, \cP}(s_h, a_h)\ge Q_{h}^{\pi, \cP}(s_{1:h}, o_{1:h}, a_{1:h}).
	\$
	It is easy to see the argument holds for $h=H$. Now note that 
	\$
	Q_{h}^{\pi^\star, \cP}(s_h, a_h)&=r_{h}(s_h, a_h)+\EE_{s_{h+1}\sim\TT_h(\cdot\given s_h, a_h)}[\max_{a_{h+1}}Q_{h+1}^{\pi^\star, \cP}(s_{h+1}, a_{h+1})]\\
	&\ge r_{h}(s_h, a_h)+\EE_{s_{h+1}\sim\TT_h(\cdot\given s_h, a_h)}[\max_{a_{h+1}}Q_{h+1}^{\pi, \cP}(s_{1:h+1}, o_{1:h+1},a_{1:h+1})]\\
	&\ge r_{h}(s_h, a_h)+\EE_{s_{h+1}\sim\TT_h(\cdot\given s_h, a_h)}[\EE_{a_{h+1}\sim\pi_{h}(\cdot\given s_{1:h+1}, o_{1:h+1},a_{1:h})}Q_{h+1}^{\pi, \cP}(s_{1:h+1}, o_{1:h+1},a_{1:h+1})]\\
	&=Q_{h}^{\pi, \cP}(s_{1:h}, o_{1:h}, a_{1:h}),
	\$
	where the first inequality comes from the inductive hypothesis.
\end{proof}

%\begin{lemma}	
%	Let $\pi^\star\in\arg\max_{\pi\in\Pi_L} v^{\cP}(\pi)$ be the best-in-class policy in $\cP$. Then by running NPG on $\hat{\cP}$, it is guaranteed that 
%	\$
%	\frac{1}{T}\sum_{t}v^{\cP}(\pi^\star)-v^{\cP}(\pi^t)\le H^2\sqrt{\frac{\log A}{T}}+SH^2\epsilon + 2\epsilon
%	\$
%\end{lemma}
%\begin{proof}
%	Note that 
%	\$
%	v^{\cP}(\pi^\star)-v^{\hat{\cP}}(\pi^t) = \sum_h\EE_{\pi^\star}^{\cP}[\langle\pi_h^\star(\cdot\given z_h)-\pi^t_h(\cdot\given z_h), Q_{h}^{\pi^t, \hat{\cP}}(s_h, z_h,\cdot)\rangle] + \EE_{\pi^\star}^\cP[Q_{h}^{\pi^t, \hat{\cP}}(s_h,z_h,a_h)-\EE^\cP_{s_{h+1}, o_{h+1}, a_{h+1}\sim\hat{\pi}}[Q_{h}^{\pi^t, \hat{\cP}}(s_{h+1}, z_{h+1},a_{h+1})]].
%	\$
%	For the first term, we have 
%	\$
%	\EE_{\pi^\star}^{\cP}&[\langle\pi_h^\star(\cdot\given z_h)-\pi^t_h(\cdot\given z_h), Q_{h}^{\pi^t, \hat{\cP}}(s_h, z_h,\cdot)\rangle]\\
%	&=\EE_{\pi^\star}^{\cP}[\langle\pi_h^\star(\cdot\given z_h)-\pi^t_h(\cdot\given z_h), \EE_{s_h\sim\tilde{b}_h^{\pi^\star}(z_h)}Q_{h}^{\pi^t, \hat{\cP}}(s_h, z_h,\cdot)\rangle]\\
%	&\le\EE_{\pi^\star}^{\cP}[\langle\pi_h^\star(\cdot\given z_h)-\pi^t_h(\cdot\given z_h), \EE_{s_h\sim\hat{b}_h^{\prime}(z_h)}Q_{h}^{\pi^t, \hat{\cP}}(s_h, z_h,\cdot)\rangle]+H\EE_{\pi^\star}^\cP[\|\hat{b}_h^{\prime}(z_h)-\tilde{b}_h^{\pi^\star}(z_h)\|_1]\\
%	&\le \EE_{\pi^\star}^{\cP}[\langle\pi_h^\star(\cdot\given z_h)-\pi^t_h(\cdot\given z_h), \EE_{s_h\sim\hat{b}_h^{\prime}(z_h)}Q_{h}^{\pi^t, \hat{\cP}}(s_h, z_h,\cdot)\rangle]+H\EE_{\pi^\star}^\cP[\|\hat{b}_h^{\prime}(z_h)-b_h^{\prime}(z_h)\|_1]+H\EE_{\pi^\star}^\cP[\|b_h^{\prime}(z_h)-\tilde{b}_h^{\pi^\star}(z_h)\|_1]\\
%	&\le \EE_{\pi^\star}^{\cP}[\langle\pi_h^\star(\cdot\given z_h)-\pi^t_h(\cdot\given z_h), \EE_{s_h\sim\hat{b}_h^{\prime}(z_h)}Q_{h}^{\pi^t, \hat{\cP}}(s_h, z_h,\cdot)\rangle]+SH\epsilon,
%	\$
%	where the last step comes from combing Lemma \ref{lem:belief}, \ref{lem:free}, and the choice of $L$.
%	Therefore, by taking average over $t\in[T]$, we have
%	\$
%	\frac{1}{T}\sum_{t\in[T]}\EE_{\pi^\star}^{\cP}[\langle\pi_h^\star(\cdot\given z_h)-\pi^t_h(\cdot\given z_h), Q_{h}^{\pi^t, \hat{\cP}}(s_h, z_h,\cdot)\rangle]&\le \EE_{\pi^\star}^{\cP}\frac{1}{T}\sum_{t\in[T]}[\langle\pi_h^\star(\cdot\given z_h)-\pi^t_h(\cdot\given z_h), \EE_{s_h\sim\hat{b}_h^{\prime}(z_h)}Q_{h}^{\pi^t, \hat{\cP}}(s_h, z_h,\cdot)\rangle]+SH\epsilon\\
%		&\le H\sqrt{\frac{\log A}{T}}+SH\epsilon.
%	\$
%	For the second term, we have
%	\$
%	\EE_{\pi^\star}^\cP&[Q_{h}^{\pi^t, \hat{\cP}}(s_h,z_h,a_h)-\EE^\cP_{s_{h+1}, o_{h+1}, a_{h+1}\sim\hat{\pi}}[Q_{h}^{\pi^t, \hat{\cP}}(s_{h+1}, z_{h+1},a_{h+1})]]\\
%	&\le \EE_{\pi^\star}^\cP[\sum_{s_{h+1}, o_{h+1}, a_{h+1}}|\PP_{h+1}^{\pi^t, \cP}(s_{h+1}, o_{h+1}, a_{h+1}\given s_{h}, z_{z}, a_{h})-\PP_{h+1}^{\pi^t, \hat{\cP}}(s_{h+1}, o_{h+1}, a_{h+1}\given s_{h}, z_{h}, a_{h})|]\\
%	&\le \EE_{\pi^\star}^\cP[\sum_{s_{h+1}, o_{h+1}, a_{h+1}}|\pi^t_h(a_{h+1}\given z_{h+1})\TT_{h}(s_{h+1}\given s_h, a_h)\OO_{h+1}(o_{h+1}\given s_{h+1})-\pi^t_h(a_{h+1}\given z_{h+1})\hat{\TT}_{h}(s_{h+1}\given s_h, a_h)\hat{\OO}_{h+1}(o_{h+1}\given s_{h+1})|]\\
%	&\le \EE_{\pi^\star}^\cP[\sum_{s_{h+1}, o_{h+1}}|\TT_{h}(s_{h+1}\given s_h, a_h)\OO_{h+1}(o_{h+1}\given s_{h+1})-\hat{\TT}_{h}(s_{h+1}\given s_h, a_h)\hat{\OO}_{h+1}(o_{h+1}\given s_{h+1})|]\\
%	&\le \EE_{\pi^\star}^\cP[\|\TT_{h}(\cdot\given s_h, a_h)-\hat{\TT}_{h}(\cdot\given s_h, a_h)\|_1 + \|\OO_{h+1}(\cdot\given s_{h+1})-\hat{\OO}_{h+1}(\cdot\given s_{h+1})\|_1]\\
%	&\le \frac{\epsilon}{H}.
%	\$
%	Therefore, by putting everything together we get
%	\$
%	\frac{1}{T}\sum_{t}v^{\cP}(\pi^\star)-v^{\hat{\cP}}(\pi^t)\le H^2\sqrt{\frac{\log A}{T}}+SH^2\epsilon + \epsilon.
%	\$
%	Meanwhile, we have
%	\$
%	|v^{\hat{\cP}}(\pi^t)-v^{\cP}(\pi^t)|\le \epsilon.
%	\$
%	Finally, we conclude that
%	\$
%	\frac{1}{T}\sum_{t}v^{\cP}(\pi^\star)-v^{\cP}(\pi^t)\le H^2\sqrt{\frac{\log A}{T}}+SH^2\epsilon + 2\epsilon
%	\$
%\end{proof}

==> Body/Hindsight.tex <==
\section{Approximate Belief Learning with Hindsight Observability \rg{(Contains Mistake)}}

\begin{definition}
    We define an algorithm $\alg$ as being $(\epsilon, \delta)$-approximate optimal with respect to a POMDP $\cP$, given a set of approximate belief states $\bb^\apx$, if it outputs a policy $\pi \in \Pi$ such that, with a probability of at least $1-\delta$, the following condition is satisfied:
    $$
    v^\cP(\pi) \geq \max_{\pi^\star\in \Pi} v^\cP(\pi^\star) - \epsilon - \sum_{h\in[H]} \EE^{\cP}_\pi\|\bb_h^\prime(z_h)-\bb_h(\tau_h)\|_1.
    $$
\end{definition}
\begin{assumption}\label{as:model-based belief learning}
We make the following assumptions about the input of \Cref{alg:hindisght-reward-free-pomdp}:
\begin{itemize}
    \item $\alg$ is $(\epsilon_0,\delta)$-approximate optimal,
    \item Our policy class $\Pi$ consists consists of policie with sufficiently long size such that for any $\gamma$-observable pomdp $\tilde{\cP}$ for each level $h\in[H]$: $$ \EE^{\tilde{\cP}}_\pi\|\bb_h(\tau_h)-\bb_h^{\apx}(z_h)\|_1\leq \epsilon_1.
	$$
\end{itemize}
    The second item of the assumption can be satisfied for a $\gamma$-observable pomdp, by using policies with quasipolynomial memory  \cite{golowich2022planning,golowich2022learning}.
\end{assumption}

\begin{algorithm}[!h]
\begin{algorithmic}
\caption{Reward-free exploration with hindsight-observability\label{alg:hindisght-reward-free-pomdp}}
\State  \textbf{Input:} \begin{itemize}
    \item hindsight access to POMDP with modifiable reward function: $$\cP(\{r_{h}\}_{h\in[H]})=(H, \cS, \cA, \cO, \{\TT_{h}\}_{h\in[H]}, \{\OO_h\}_{h\in[H]}, \mu_1, \{r_{h}\}_{h\in[H]}),$$
    \item Algorithm $\alg(\hat{\cP})$ that takes as input a POMDP $\hat{\cP}$ with $H^*$ levels, and a set of approximate beliefs $\{\hat{\bb}_h\}_{h\in[H^*]}$ and computes an approximate optimal policy,  
    \item total number of trajectories $K$ per level-state-action triplet.
\end{itemize}
\State Initialize approximate belief: $\bb^\apx_0=\emptyset$.
\For{$H^*\in[H]$}
\For{$s_h\in\cS$, and $a_h\in \cA$}
	\State $\hat{r}_{h^\prime}(s_h^\prime, a_h^\prime)\leftarrow \mathbbm{1}[h^\prime=H^*, s_h^\prime=s_h,a_h^\prime = a_h]$ for any $h^\prime, s_h^\prime, a_h^\prime\in[H^*]\times\cS\times\cA$.
	\State $\Psi(h, s_h,a_h)\leftarrow \alg(\cP(\{\hat{r}_{h}\}_{h\in[H^*]},\{\bb_h^\apx\}_{h\in[H^*-1]}))$.
 \State \Comment{See \Cref{obs:belief up to previous level} to see why approximate beliefs up to level $H^*-1$ suffice.}
    \State Collect $K$ trajectories $\{(s_h^i, o_{h}^i, a_h^i, s_{h+1}^i)\}_{i\in[K]}$ using policy $\Psi(h, s_h,a_h)$, and consider the dataset: $$\DD_{(h,s_h,a_h)} = \{(s_h^i, o_{h}^i, a_h^i, s_{h+1}^i):\text{ $i\in[K]$ and $s_{h}^i=s_h$ }\}.$$
\EndFor
\State Update approximate belief:
$$\bb_{H^*}^\apx=\Cref{alg:belief learning from datasets}\left(\left\{\DD_{(h,s_h,a_h)}\right\}_{h\in[H^*]}\right) \text{ with $\epsilon_0=\rg{...}$}$$
\EndFor
\State \Return 
\end{algorithmic}

\end{algorithm}

\begin{observation}\label{obs:belief up to previous level}
    %Given a reward-free pomdp $\cP=(H, \cS, \cA, \cO, \{\TT_{h}\}_{h\in[H]}, \{\OO_h\}_{h\in[H]}, \mu_1)$, for fixed level $H^*\in[H]$, consider the auxiliary $\hat{\cO}:=\{o_{s}\}_{s\in \cS}$, and the latent-state revealing emission $\hat{\OO}_{H^*}(o \given s)=\ind[o=o_s]$, where for state $s\in \cS$, we denote by $o_s$ the corresponding element in $\hat{\cO}$. 
    
    
    
    %Consider the auxilliary pomdp $$\tilde{\cP}=(H^*, \cS, \cA, \cO\cup \hat{\cO}, \{\TT_{h}\}_{h\in[H^*]}, \{\OO_h\}_{h\in[H^*-1]}\cup \tilde{\OO}_{H^*}, \mu_1,),$$ that is, pomdp $\tilde{\cP}$ has the same distribution over transition like the pomdp $\cP$ up to level $H^*-1$, with the difference that at level $H^*$ pomdp $\tilde{\cP}$ reveals the latent state $s_{H^*}$ and terminates at the next iteration.



    Consider a reward-free POMDP, denoted by $\cP = (H, \cS, \cA, \cO, \{\TT_{h}\}_{h\in[H]}, \{\OO_h\}_{h\in[H]}, \mu_1)$. For a specified level $H^* \in [H]$, introduce an auxiliary observation set $\hat{\cO} := {o_{s}}{s\in \cS}$, and define a latent-state revealing emission model for the $H^*$ level as $\hat{\OO}_{H^*}(o \given s) = \ind[o=o_s]$, where $o_s$ is the unique observation in $\hat{\cO}$ corresponding to state $s \in \cS$.

Construct an auxiliary POMDP, $\tilde{\cP} = (H^, \cS, \cA, \cO \cup \hat{\cO}, \{\TT_{h}\}_{h\in[H^]}, \{\OO_h\}_{h\in[H^*-1]} \cup \tilde{\OO}_{H^*}, \mu_1)$. Observe that:
\begin{itemize}
    \item The transition dynamics $\TT_{h}$ and observation models $\OO_h$ for levels up to $H^*-1$ are inherited from $\cP$ without modification. At level $H^*$, $\tilde{\cP}$  reveals the latent state $s_{H^*}$ via the observation $o_s$ and concludes the episode in the subsequent step. 
    \item If pomdp $\cP$ is $\gamma$-observable, then pomdp $\tilde{\cP}$ is also $\gamma$-observable.
    \item For any policy $\pi\in \Pi$, we can simulate one trajectory for pomdp $\tilde{\cP}$ using one trajectory of pomdp $\cP$.
\end{itemize}

For fixed state $s_{H^*}\in \cS$ and action $a_{H^*}\in \cA$, consider the reward function that only awards when the agent is at latent state $s_{H^*}$ at level $H^*$, and takes action $a_{H^*}$, e.g.
$$r_h(s_h,a_h) = \ind[h=H^*,s_h=s_{H^*},a_h=a_{H^*}],
$$
and consider the problem of finding an approximately-optimal policy for pomdp $\cP$ coupled with reward $\{r_h\}_{h\in[H]}$ when the agent has approximate beliefs $\{\bb^\apx_h\}_{h\in[H^*-1]}$ only for the $H^*-1$ levels.


Then given an output $\pi$ of an $(\epsilon,c,\delta)$-precision algorithm on pomdp $\tilde{\cP}$ with augmented approximate belief $\{\bb^\apx_h\}_{h\in[H^*-1]}\cup \{\bb^\apx_{H^*}(s\given o_{s'})=\ind[s=s']\}$, then we can construct policy $\pi'\in \Pi$ such that with probability at least $1-\delta$:
$$
v^\cP(\pi') \geq \max_{\pi^*\in \Pi} v^\cP(\pi^\star) - \epsilon - c\cdot\sum_{h\in[H^*-1]} \EE^{\cP}_\pi\|\bb_h(\tau_h)-\bb_h^{\apx}(z_h)\|_1.\footnote{\text{The modified policy $\pi'$ always picks action $a_{H^*}$ at level $H^*$ disregarding the observant.}}
$$


\end{observation}

\begin{algorithm}[!h]
\begin{algorithmic}
\caption{Belief-Learning from Datasets}\label{alg:belief learning from datasets}

\State  \textbf{Input:} \begin{itemize}
    \item Target level $H^*$ we want to learn the belief, precision parameter $\epsilon_0> 0$ , homing parameter $\eta$, and probability level $\delta\in(0,1)$.
    \item For each level $h\in[H^*]$, state $s_h\in \cS$ and action $a\in \cA$, a dataset constainting samples from $\OO(\cdot\given s_h)$ and $\TT(\cdot\given s_h,a_h)$: $\DD_{(h,s_h,a)}$
\end{itemize}
\State Set threshold parameter $N \leftarrow \frac{254\cdot H^2\cdot \left(\max(|\cA|,|\cO|)+ 2 \log(2/\delta)\right)}{\epsilon_0^2}$ 
\State Define auxiliarry state and observation $s_{exit}$, $o_{exit}$.
\State For $h\in[H^*-1]$, define $\hat{\cS}_h=\{s_h\in \cS: |\DD_{(h,s_h,a_h)}|\geq N, \forall a\in \cA \}$.

\For{$h\in[H^*-1]$,$s_h\in \hat{\cS}_h$, $a\in \cA$}
    \State $N_{h}(s_h, o_{h})\leftarrow \sum_{a\in\cA}\sum_{o_h'\in \DD_{(h,s_h,a)]}}\mathbbm{1}[o_h'=o_h]$ for any $o_{h}\in\cO$
    \State $N_{h}(s_h, a, s_{h+1})\leftarrow \sum_{s_{h+1}'\in \DD_{(h,s_h,a)]}}\mathbbm{1}[s_{h+1}'=s_{h+1}]$ for any $a\in\cA$
    \State $\hat{\OO}_h(o_h\given s_h)=\begin{cases}\frac{ N_h(s_h, o_h)}{\sum_{o_h'\in\cO}N_h(s_h, o_h)} \qquad&\text{for any $s_h\in\hat{\cS}_h$ and $o_{h}\in\cO$,}\\
    \ind[o_h=o_{exit}] &\text{if $s_{h}=s_{exit}$.}
    \end{cases}$.
    \State $\hat{\TT}_h(s_{h+1}\given s_h,a)=\begin{cases} \frac{N_h(s_h, a, s_{h+1})}{\sum_{a'\in\cA}N_h(s_h, a', s_{h+1})}\qquad & \text{for any $s_h\in \hat{\cS}_h, s_{h+1}\in\hat{\cS}_{h+1}$},\\
    1-\sum_{s_{h+1}'\in \hat{\cS}_{h+1}}\frac{N_h(s_h, a, s'_{h+1})}{\sum_{a'\in\cA}N_h(s_h, a', s_{h+1})}\qquad & \text{for any $s_h\in \hat{\cS}_h, s_{h+1}=s_{exit}$},\\
    \ind[s_{h+1}=s_{exit}] & \text{ if $s_{h}=s_{exit}$.}
    \end{cases}$ .
    
\EndFor
\State
\State \Return approximate belief $\bb^{\prime}_{H^*}(\cdot)$ according to transition matrices $\{\hat{\TT}_h\}_{h\in[H^*]}$ and emission matrix $\{\hat{\OO}_h\}_{h\in[H^*]}$.
\end{algorithmic}
\end{algorithm}

\begin{definition}[\rg{Remdmber to cite original paper}]
    Consider a POMDP instance $\cP$. A policy $\pi\in \Pi$ is $\eta$-homing for state $s_h\in \cS$ at level $h\in[H]$ if $
    \PP^{\pi, \cP}( s'_{h}=s_h)\geq \eta.$ Moreover, we denote the set of $\eta$-homing states at level $h\in[H]$ by:
\$
	\cS^{\eta}_h:=\{s_h\in\cS\given \text{$\exists$  $\eta$-homing policy $\pi\in \Pi$ for state $s_h$ at level $h$.} \}.
	\$
\end{definition}
\begin{theorem}\label{lem:belief}
\rg{TODO}
Under \Cref{as:model-based belief learning}, if for each level $h\in[H]$, state $s_h\in \cS_h^{\eta}$, and action $a\in \cA$, dataset $\DD_h$ (c.f. \Cref{alg:belief learning from datasets}) was collected using an $\frac{\eta_h}{C_h}$-Homing policy, for some $C_h\geq 1$ with at least \rg{$K\geq\frac{1}{\eta_h} \max\left(2\cdot C_h \cdot N, 4\log(\delta) \right)$} total attempts, then with probability at least $1-\delta \cdot|\cA|\cdot |\cS| \cdot H$:
\$
	&\EE^{\cP}_\pi\|\bb_H(\tau_H)-\hat{\bb}_H^{\prime,\trunc}(z_H)\|_1\le \epsilon_0 + \epsilon_1 + 18 \rg{|\cS|} \sum_{h\in[H-1]}  \eta_h .
	\$


\end{theorem}

\begin{proof}
	To simplify calculations set $\kappa = \frac{\epsilon_0}{16\cdot H}$.  To prove approximation guarantees we make repeated use of \Cref{lem:traj}. The key challenge for the proof is that there could exist some states $s_h$ at level $h$ that can only be visited with a low probability no matter what exploration policy is used. To circumvent this issue, our key technique here is to contruct a proxy POMDP where we \emph{ignore} the transition into states that cannot be explored sufficiently. Therefore, emission at such states may not be learned accurately. We show in the following fact that the set of states $\hat{\cS}_h$, contains any state that can be explored for some sufficient probability.
    \begin{fact}\label{fact:visit frequent states}
        For each level $h$, with probability at least $1 - |\cA|\cdot |\cS|\cdot H\cdot \delta$, $\cS_h^{\eta} \subseteq \hat{\cS}_h$.
    \end{fact}
    \begin{proof}
    For fixed level $h\in[H]$, state $s_h\in \cS^{\eta}_h$, we calculate the probability that $s_h\notin\hat{\cS}_h$. Since $s_h\in \cS^{\eta}_h$, the samples in datasets $\DD_{(h,s_h)}:=\cup_{a\in\cA}\DD_{(h,s_h,a)}$ were collected using a policy that guarantees visiting state $s_h$ at level $h\in[H]$ with probability at least $\frac{\eta}{C}$, and there a total of $K$ attempts for each action $a\in \cA$:
    $$\E_{\DD_{(h,s_h,a)}}\left[|\DD_{(h,s_h,a)}| \right] \geq \frac{\eta\cdot K}{C}.$$ 
    By Chernoff bound, since $K\geq \frac{2\cdot C \cdot N}{\eta}$ the probability that state $s_h$ is not in $\hat{\cS}_h$ is at most:
            $$
\sum_{a\in \cA}\Pr\left[|\DD_{(h,s_h,a)}| < N \right]\leq |\cA|\cdot \Pr\left[|\DD_{(h,s_h,a)}| <  \frac{\eta\cdot  K}{2\cdot C} \right]\leq |\cA|\cdot e^{-\frac{\eta\cdot K }{4\cdot C}} \leq |\cA|\cdot e^{-\frac{\eta\cdot K }{4}} \leq |\cA|\cdot  \delta.
            $$
        The rest of the proof follows by Union-Bound for each level $h\in[H]$ and state $s_h\in \cS$.

        \notshow{Now we prove that with probability at least $1 - |\cS|\cdot H\cdot \delta$, $\cS_h^{\eta}$, $\hat{\cS}_h \subseteq \cS_h^{\frac{\eta}{8}}$. The proof follows similar to the previous case. For fixed level $h\in[H]$ and state $s_h\notin \cS^{\frac{\eta}{8}}_h$. The samples in datasets $\DD_{(h,s_h)}:=\cup_{a\in\cA}\DD_{(h,s_h,a)}$ were collected using a policy that guarantees visiting state $s_h$ at level $h\in[H]$ with probability at most $\frac{\eta}{8}$, and thus: $$\E_{\DD_{(h,s_h)}}\left[\sum_{(s'_h,o'_h,a'_h,s'_{h+1})\in \DD_{(h,s_h)}} \ind[s'_h = s_h]\right] \leq \frac{\eta\cdot |\cA|\cdot N}{8}.$$ By Chernoff bound, the probability that state $s_h$ is in $\hat{\cS}_h$ is at most: $$\Pr\left[\sum_{(s'_h,o'_h,a'_h,s'_{h+1})\in \DD_{(h,s_h)}} \ind[s'_h = s_h] > \frac{\eta\cdot |\cA|\cdot N}{4} \right]\leq e^{-\frac{\eta\cdot|\cA|\cdot N}{24}} \leq \delta.
            $$
        The rest of the proof follows by Union-Bound for each level $h\in[H]$ and state $s_h\in \cS$.
        }
    \end{proof}


 
 
 

    We condition on \Cref{fact:visit frequent states} for the rest of the proof, which happens with probability at least $1-\delta \cdot |\cS|\cdot |\cA|\cdot H$. Now we are ready to construct a pomdp containing only the states that we can explore with sufficient probability and an additional dummy state $s_{exit}$ and observation $o_{exit}$, and we use as proxy for our analysis. Formally, we define a pomdp $\cP^\trunc$ with state space for each level $h\in[H]$ and observation space: 
	\$ \cS_h^{\text{trunc}}:=\hat{\cS}_h\cup \{s_{exit}\},\quad 
	\cO^{\text{trunc}}:=\cO\cup \{o_{exit}\}.
	\$
	For transition, we define for each level $h\in[H]$, states $s_h\in \cS_h^\trunc$, $s_{h+1}\in \cS_{h+1}^\trunc$ and action $a\in cA$:
$$
	\TT_h^{\text{trunc}}(s_{h+1}\given s_h, a_h) =\begin{cases} \TT_{h}(s_{h+1}\given s_h, a_h) \qquad&\text{if $s_h\in \hat{\cS}_h, s_{h+1}\in \hat{\cS}_{h+1}$}, \\
 1-\sum_{s_{h+1}\in\hat{\cS}_{h+1}  } \TT_{h}(s_{h+1}\given s_h, a_h) & \text{if $s_h\in \hat{\cS}_h,s_{h+1}=s_{exit}$,}\\
 \ind[s_{h+1}=s_{exit}] & \text{if $s_h=s_{exit}$.}
 \end{cases}
$$
	 For emission, we define
	\$
	\OO_{h}^{\text{trunc}}(o_h\given s_{h}):=\begin{cases}
            \ind[o_h=o_{exit}] \qquad\qquad&\text{if $s_h=s_{exit}$},\\
	    \OO_{h}(o_h\given s_h), & \text{if $s_h\in\hat{\cS}_{h}$.}
	\end{cases}
	\$

    \notshow{Now we examine the total variation distance of trajectory distribution in $\cP$ and $\cP^\trunc$.
	For any policy $\pi\in\Pi^{\text{gen}}$, it is easy to see that
	\$
	\PP^{\pi, \cP}(\overline{\tau}_H)=\PP^{\pi, \cP^\trunc}(\overline{\tau}_H)
	\$
	for any $\overline{\tau}_H\in\overline{\cT}_H^{\high}:=\{(s_{1:H}, o_{1:H}, a_{1:H})\given s_{h}\in\hat{\cS}_h, \forall h\in[H]\}$. Meanwhile, by Union bound and since \rg{$\cS_h^{\eta}\subseteq \hat{\cS}_h$} it holds that:
	\$
	\PP^{\pi, \cP}(\overline{\tau}_H\not\in\overline{\cT}_H^{\high})\le \sum_{h}\PP_h^{\pi, \cP}(s_h\notin\hat{\cS}_h)\le H\cdot |S|\cdot \rg{\eta}.
	\$
 }
	By \Cref{lem:traj} the total variation distance of trajectory distribution in $\cP$ and $\cP^\trunc$ and beliefs can be bound by 
 \begin{align*}
     \EE_{\pi}^{\cP}[\|\bb_h(\tau_h)-\bb_h^{\trunc}(\tau_h)\|_1]&\le 2\cdot \EE_{\pi}^{\cP}\left[\sum_{h\in[H]}\|\TT_{h}(\cdot\given s_h, a_h)-\TT^\trunc_{h}(\cdot\given s_h, a_h)\|_1+\|\OO_{h}(\cdot\given s_h)-\OO^{\trunc}_{h}(\cdot\given s_h)\|_1\right]\\
	&\le 4\cdot \sum_{h\in[H-1]}  \PP^{\pi, \cP}( s_{h+1}\not\in\hat{\cS}_{h+1}) + 2\cdot \sum_{h\in[H]}\PP^{\pi, \cP}( s_h\not\in\hat{\cS}_h)\\
	&\le 6\cdot \sum_{h\in[H]}  \eta_h,\\
 \sum_{\overline{\tau}_H}|\PP^{\pi, \cP}(\overline{\tau}_H)-\PP^{\pi, \cP^\trunc}(\overline{\tau}_H)|&\le  \EE_{\pi}^{\cP}\left[\sum_{h\in[H]}\|\TT_{h}(\cdot\given s_h, a_h)-\TT^\trunc_{h}(\cdot\given s_h, a_h)\|_1+\|\OO_{h}(\cdot\given s_h)-\OO^{\trunc}_{h}(\cdot\given s_h)\|_1\right]\\
 &\le 3\cdot \sum_{h\in[H]}  \eta_h.
 \end{align*}

    Thus proxy pomdp $\cP^{\trunc}$ serves as an accurate proxy for the real podmp $\cP$. For the remaining of the proof, we show that the output of \Cref{alg:belief learning from datasets} learns accurately the belief $\bb_h^{\trunc}(\tau_h)$.


    
    Observe that for each level $h\in[H]$, and state $s_h\in \hat{\cS}_h$ in \Cref{alg:belief learning from datasets}, with probability at least $1-\delta$, the estimated emission matrix $\hat{\OO}_h(\cdot \mid s_h)$ and for each action $a\in \cA$ the transition matrix $\hat{\TT}_h(\cdot \mid s_h, a)$ satisfies for each level $h\in[H]$ and state $s_h\in \hat{\cS}_h$ \citep{canonne2020short}: 
    \begin{align*}
        \|\OO_h^{\trunc}(\cdot\given s_h)-\hat{\OO}_h(\cdot\given s_h)\|_1=\|\OO_h(\cdot\given s_h)-\hat{\OO}_h(\cdot\given s_h)\|_1\leq \frac{\kappa}{\sqrt{|\cA|}}, \\ \|\TT^{\trunc}_h(\cdot\given s_h,a)-\hat{\TT}_h(\cdot\given s_h,a)\|_1\leq  \|\TT_h(\cdot\given s_h)-\hat{\TT}_h(\cdot\given s_h,a)\|_1\leq \kappa
    \end{align*}
	
	Now we are ready to examine $\hat{\bb}_h^{\prime, \trunc}$. Since for any level $h$ and state $s_h\in \hat{\cS}_h$, $\OO(\cdot\given s_h)=\OO^{\trunc}(\cdot\given s_h)$, and additionally $\OO^\trunc(o_h\given s_{exit}) = \ind[o_h=o_{exit}]$ then $\cP^\trunc$ is $\gamma$-observable, \Cref{as:model-based belief learning}, it holds that 
	\$
	\EE^{\hat{\cP}^\trunc}_\pi\|\hat{\bb}_h^{\trunc}(\tau_h)-\hat{\bb}_h^{\prime,\trunc}(z_h)\|_1 \leq \epsilon_1.
	\$

    Now we show that under the assumptions of the theorem, \Cref{alg:belief learning from datasets} learns POMDP $\cP^{\trunc}$. Hence, by Lemma \ref{lem:traj}, it holds that for the total variation distance of trajectory distributions between $\cP^\trunc$ and $\hat{\cP}^\trunc$, it holds that
    \begin{align*}
	\EE^{\cP^\trunc}_\pi\|\bb_h^{\trunc}(\tau_h)-\hat{\bb}^\trunc_h(\tau_h)\|_1&\le2\left(\EE_{\pi}^{\cP^\trunc}\sum_{h}\|\TT^\trunc_{h}(\cdot\given s_h, a_h)-\hat{\TT}_{h}(\cdot\given s_h, a_h)\|_1+\|\OO_{h}(\cdot\given s_h)-\hat{\OO}^\trunc_{h}(\cdot\given s_h)\|_1\right) \\ 
 &\leq4\cdot H \cdot \kappa,\\
 \sum_{\overline{\tau}_H}|\PP^{\pi, \cP^\trunc}(\overline{\tau}_H)-\PP^{\pi, \hat{\cP}^\trunc}(\overline{\tau}_H)|&\le \EE_{\pi}^{\cP^\trunc}\sum_{h}\|\TT^\trunc_{h}(\cdot\given s_h, a_h)-\hat{\TT}_{h}(\cdot\given s_h, a_h)\|_1+\|\OO_{h}(\cdot\given s_h)-\hat{\OO}^\trunc_{h}(\cdot\given s_h)\|_1\\
	&\leq 2\cdot H \cdot \kappa.\\
	    \end{align*}

	Finally, we conclude byare ready to prove
	\$
	&\EE^{\cP}_\pi\|\bb_h(\tau_h)-\hat{\bb}_h^{\prime,\trunc}(z_h)\|_1\\
 \le& \EE^{\cP}_\pi\|\bb_h(\tau_h)-\bb_h^{\trunc}(\tau_h)\|_1+\EE^{\cP}_\pi\|\bb_h^{\trunc}(\tau_h)-\hat{\bb}^\trunc_h(\tau_h)\|_1+\EE^{\cP}_\pi\|\hat{\bb}^\trunc_h(\tau_h)-\hat{\bb}^{\prime, \trunc}_h(z_h)\|_1\\
	\le &\EE^{\cP}_\pi\|\bb_h(\tau_h)-\bb_h^{\trunc}(\tau_h)\|_1+\EE^{\cP^\trunc}_\pi\|\bb_h^{\trunc}(\tau_h)-\hat{\bb}^\trunc_h(\tau_h)\|_1+\EE^{\hat{\cP}^\trunc}_\pi\|\hat{\bb}^\trunc_h(\tau_h)-\hat{\bb}^{\prime, \trunc}_h(\tau_h)\|_1 \\
	&\quad\quad+ 4\|\PP^{\pi, \cP}-\PP^{\pi, \cP^\trunc}\|_1+2\|\PP^{\pi, \cP^\trunc}-\PP^{\pi, \hat{\cP}\trunc}\|\\
	&\le 6\cdot\sum_{h\in[H]}  \eta_h + 4\cdot H \cdot \kappa    +12\cdot\sum_{h\in[H]}  \eta_h + 4\cdot H \cdot \epsilon_1\\
	&\le 18 \sum_{h\in[H]}  \eta_h + 8 \cdot H \cdot \kappa + \epsilon_1 \\
 &\leq 18 \sum_{h\in[H]}  \eta_h + \epsilon_0 + \epsilon_1.
	\$
\end{proof}

\rgn{THe theorem below is wrong.}
\begin{theorem}\label{lem:belief}

Let $\{\bb_h^{\prime}\}_{h\in[H]}$ be the outcome of \Cref{alg:hindisght-reward-free-pomdp} when $\alg$ is $(\frac{\eta}{4},\delta)$. If \Cref{as:model-based belief learning} and $K\geq \frac{8}{\eta}\max\left( |\cA|,|\cO|, \log(2/\delta)\right)$, then with probability at least $1-...$ for any policy $\pi\in\Pi$ and level $h\in[H]$:
$$
\EE^{\cP}_{\tau\sim\pi} \|\bb_h(\tau_h)-\bb_h^{\prime}(z_h) \|_1\le \frac{\eta}{4\cdot H}
$$
\end{theorem}
\begin{proof}
    We prove that for when $h\in[H]$, with probability at least $1-\rg{...}$, . The base case $h=0$ holds trivially with probability $1$.

    Assume that when \Cref{alg:hindisght-reward-free-pomdp} is at level $H^*\geq 1$, with probability at leas $1-\rg{...}$:
    $$\EE^{\cP}_{\tau\sim\pi} \|\bb_h(\tau_h)-\bb_h^{\prime}(z_h) \|_1\le \frac{\eta}{4\cdot H} \qquad\qquad \forall h\in[H^*-1].$$

    During level $H^*$, $\alg$ is executed a total of $|\cA|\cdot|\cS|$ times, and since $\alg$ is $(\frac{\eta}{4},\delta)$-optimal, with probability at least $1-|\cA|\cdot|\cS|\cdot \delta$, for each state $s_h\in \cS_h^{\eta}$ and action $a_h\in \cA$,  policy $\Psi(h,s_h,a_h)$ satisfies:
    $$
    \PP^{\pi, \cP}( s'_{h}=s_h) \geq \frac{\eta}{2}.
    $$

    Moreover since $K\geq \frac{8}{\eta}\max\left( |\cA|,|\cO|, \log(2/\delta)\right)$, by \Cref{lem:belief} with probability at least $1-\delta\cdot |\cA|\cdot|\cS|\cdot h$:
    $$
\EE^{\cP}_{\tau\sim\pi} \|\bb_h(\tau_h)-\bb_h^{\prime}(z_h) \|_1\le \frac{\eta}{4\cdot H},
$$
which concludes teh proof.
\end{proof}


==> Body/POSG-Reward-Free.tex <==
\section{Preliminaries for POSG}
\subsection{POSG with information sharing}
\paragraph{Model.}
Formally, we define a POSG with $n$ agents by a tuple $\cG = (H, \mathcal{S}, \{\mathcal{A}_i\}_{i=1}^{n}, \{\mathcal{O}_i\}_{i=1}^{n}, \mathbb{T}, \mathbb{O}, \mu_1, \{r_i\}_{i=1}^{n})$, where $H$ denotes the length of each episode, $\mathcal{S}$ is the state space with $|\mathcal{S}|=S$, $\mathcal{A}_i$ denotes the action space for the $i^{th}$ agent with $|\mathcal{A}_i|=A_i$. We denote by $a := (a_1, \cdots, a_n)$ the joint action  of all the $n$ agents, and by $\mathcal{A}=\mathcal{A}_1\times \cdots\times \mathcal{A}_n$ the joint action space with $|\mathcal{A}| = A=\prod_{i=1}^{n}A_i$. We use $\mathbb{T}=\{\mathbb{T}_h\}_{h\in [H]}$ to denote the collection of the transition matrices, so that $\mathbb{T}_h(\cdot\given s, {a})\in\Delta({\mathcal{S}})$ gives the probability of the next state if joint action ${a}$ is taken at state $s$ and step $h$. In the following discussions, for any given $a$, we treat $\TT_h(a)\in\RR^{|\cS|\times|\cS|}$ as a matrix, where each row gives the probability for the next state.  {We use} $\mu_1$ {to} denote the distribution of the initial state $s_1${, and} $\cO_i$ {to} denote the observation space for the $i^{th}$ agent with $|\mathcal{O}_i|=O_i$.  We denote by ${o}:=(o_1, \dots, o_n)$ the joint observation of all $n$ agents, and by $\mathcal{O}:=\mathcal{O}_1\times\dots\times\mathcal{O}_n$ with $|\mathcal{O}|=O=\prod_{i=1}^{n}O_i$. We use $\mathbb{O}=\{\mathbb{O}_h\}_{h\in [H + 1]}$ to denote  the collection of the joint emission matrices, so that $\mathbb{O}_h(\cdot\given s)\in\Delta({\mathcal{O}})$ gives the emission distribution over the joint observation space $\mathcal{O}$ at state $s$ and step $h$.  {For notational convenience, we will at times adopt the matrix convention, where $\OO_h$ is a matrix with rows $\OO_h(\cdot\given s_h)$.} We also denote $\OO_{i, h}(\cdot\given s)\in \Delta(\cO_i)$ as the marginalized emission for the $i^{th}$ agent. Finally, $r_i=\{r_{i, h}\}_{h\in [H + 1]}$ is a collection of reward functions, so that $r_{i, h}(s_h, a_h)$ is the reward of {the} $i^{th}$ agent given the state $s_h$ and joint action $a_h$ at step $h$. 

Similar to POMDO, in a POSG, the states are always hidden from agents, and each agent can only observe its own individual observations. The game proceeds as follows.  At the beginning of each episode, the environment samples $s_1$ from $\mu_1$. At each step $h$, each agent $i$ observes its own observation $o_{i, h}$, where ${o}_h:=(o_{1, h},\dots, o_{n, h})$ is sampled jointly from $\mathbb{O}_h(\cdot\given  s_h)$. Then each agent $i$ takes the action $a_{i, h}$ and receives the reward $r_{i,h}(s_h, a_h)$. After that the environment transitions to the next state $s_{h+1}\sim \mathbb{T}_h(\cdot\given s_h, {a}_h)$. The current episode terminates immediately once $s_{H+1}$ is reached. 

% \vspace{-10pt}
\paragraph{Information sharing, common and private information.} 
Each agent $i$ in the POSG maintains its own information,  $\tau_{i, h}$, a collection of historical observations and actions  at step $h$, namely,  $\tau_{i, h} \subseteq \{o_1, a_{1}, o_2, \cdots, a_{h-1}, o_{h}\}$, and the collection of the history at step $h$ is given by $\mathcal{T}_{i, h}$.  
%\kz{might be better to specify what's in $\tau_{i, h}$, i.e., $\tau_{i, h}=\{a_{i,1}, o_{i,2}, \cdots, a_{i,h-1}, o_{i,h}\}\subseteq \{a_{1}, o_2, \cdots, a_{h-1}, o_{h}\}$? in case people may think it is just ANY  SUBSET. also, maybe introduce $\tau_{h}$ here, and define it to be the whole history $\{a_{1}, o_2, \cdots, a_{h-1}, o_{h}\}$.}\xy{I think it is any subset}

% The joint history is given by ${\tau}_h := (\tau_{1, h}, \dots, \tau_{n, h})$ and the collection of joint history is given by $\mathcal{T}_h = \mathcal{T}_{1, h}\times\cdots\times\mathcal{T}_{n, h}$. 

{In many practical examples, agents may share part of the history with each other, which may introduce more structure in the game that leads to both sample and computation efficiency. The information sharing splits  the history into \emph{common/shared} and \emph{private}  information for each agent.} 
The \emph{common information} at step $h$ is a subset of the joint history $\tau_h$: ${c}_h \subseteq \{o_1, a_{1}, o_2, \cdots, a_{h-1}, o_{h}\}$, which is available to \emph{all the agents} in the system, and the collection of the common information is denoted as $\cC_h$ and  we define $C_h=|\cC_h|$. Given the common information ${c}_h$, each agent also has the private information $p_{i, h} = \tau_{i, h}\setminus{c_h}$, where the collection of the private information for the $i^{th}$ agent is denoted as $\cP_{i, h}$ and its  cardinality as  $P_{i, h}$. The joint private information at step $h$ is denoted as $p_{h}$, where the collection of the joint private history is given by $\cP_h = \cP_{1, h}\times\cdots\times\cP_{n, h}$ and the corresponding cardinality is $P_{h} = \prod_{i=1}^nP_{i, h}$. We allow $c_h$ or $p_{i, h}$ to take the special value $\emptyset$ when there is no  common or private information. {In particular, when $\cC_h = \{\emptyset\}$, the problem reduces to the general POSG without any favorable information structure; when $\cP_{i, h} = \{\emptyset\}$, every agent holds the same history, and it reduces to a POMDP when the agents share a common reward function and the goal is usually to find the team-optimal solution.} 

{Throughout,} we also assume that the common information and private information evolve over time properly. 

\begin{assumption}[Evolution of common and private information]\label{evo}
We assume that common information and private information evolve over time as follows:
\begin{itemize}
    \item Common information $c_h$ is non-decreasing with time, that is, $c_h\subseteq c_{h+1}$ for all $h$. Let $z_{h+1} = c_{h+1}\setminus c_h$. Thus, $c_{h+1}=\{c_h, z_{h+1}\}$. Further, we have 
   \begin{align}\label{common_trans}
        z_{h+1} = \chi_{h+1}(p_h, a_h, o_{h+1}),
    \end{align}
    where $\chi_{h+1}$ is a fixed transformation. We use $\cZ_{h+1}$ to denote the collection of $z_{h+1}$ at step $h$. 
    \item Private information evolves according to: 
    \begin{align}\label{private_trans}
        p_{i, h+1} = \xi_{i, h+1}(p_{i, h}, a_{i, h}, o_{i, h+1}),
    \end{align}
    where $\xi_{i, h+1}$ is a fixed transformation.
\end{itemize}
\end{assumption} 

Equation \eqref{common_trans} states that the increment in the common information depends on the ``new" information $(a_h, o_{h+1})$ generated between steps $h$ and $h+1$ and part of the old information $p_h$. {The incremental common information can be implemented by certain sharing and communication protocols among the agents.} Equation \eqref{private_trans} implies that the evolution of private information only depends on the newly generated private information $a_{i, h}$ and $o_{i, h+1}$. These evolution rules are standard in the literature \citep{nayyar2013common, nayyar2013decentralized}, specifying the source of common information and private information. {Based on such evolution rules, we define $\{f_h\}_{h\in [H+1]}$ and $\{g_h\}_{h\in [H+1]}$, where $f_h:\cA^h\times\cO^h\rightarrow \cC_h$ and $g_h:\cA^h\times\cO^h\rightarrow \cP_h$ for $h\in [H+1]$, as the mappings that map the joint history to common information and joint private information, respectively.}

\subsection{Policies and value functions}
We define a stochastic policy for the $i^{th}$ agent at step $h$ as: 
\begin{align}\label{policygame}
    {\pi}_{i, h}: \Omega_h\times\cP_{i, h}\times \cC_{h}\rightarrow \Delta({\mathcal{A}_i}).
\end{align}
The corresponding policy class is denoted as ${\Pi}_{i, h}$. {Hereafter, unless otherwise noted, when referring to \emph{policies}, we mean the policies given in the form of \eqref{policygame}, which maps the available information of the $i^{th}$ agent, i.e., the private information together with the common information, to the distribution over her actions.} Here {$\omega_{i, h}\in \Omega_h$ is the random seed, and $\Omega_h$ is the random seed space, which is shared among agents.} We further denote $\Pi_i = \times_{h\in [H]} \Pi_{i, h}$ as the policy space for agent $i$ and $\Pi$ as the joint policy space. 
As a special case, we define the {space of}  
\emph{deterministic}  policy {as $\Tilde{\Pi}_i$, where $\Tilde{\pi}_i\in\Tilde{\Pi}_i$} maps the private information and common information to a \emph{deterministic} action for the $i^{th}$ agent and the joint space as $\Tilde{\Pi}$.
%\kz{change back to product notation.}
%%\small
%\$
%\Tilde{\pi}_{i, h}: \cP_{i, h}\times\cC_h\rightarrow \cA_i.
%\$
%%\normalsize 
%We denote the corresponding policy class as $\Tilde{\Pi}_{i, h}$. Furthermore, the deterministic policy for the $i^{th}$ agent is denoted as $\Tilde{\pi}_i = ({\Tilde{\pi}_{i, h}})_{h=1}^{H}$, and the corresponding class is $\Tilde{\Pi}_{i}$. 

One important  concept   in 
the {common-information-based   framework} 
% partially observable domain 
is called the \emph{prescription} \citep{nayyar2013decentralized,nayyar2013common}, defined for the $i^{th}$ agent as
%\kz{actually, this two-step policy is ``less representative'' than general joint and correlated policy that can be represented by \eqref{policy}, right (since the choice of this $\gamma$ is correlated, but the further mapping to $\Delta(\cA_i)$ is definitely product policy and thus not correlated, right?)? lets talk.}
%\kz{maybe 1-2 sentences explaining what this function really is? now it is a bit abrupt, and this is a new concept to ML people.}
% \kz{define $\Gamma_{i, h}$ as the function class here, and $\Gamma$ as the collection of all of them.}
$
\gamma_{i, h}: \cP_{i, h}\rightarrow \Delta(\cA_i).
$ 
With such a prescription function, agents can take actions purely based on their local private information. We define $\Gamma_{i, h}$ as the function class for prescriptions, and $\Gamma:=\{\Gamma_{i, h}\}_{i\in [n], h\in [H]}$ as the function class for  joint prescriptions. Intuitively, the partial function $\pi_{i, h}(\cdot\given\omega_{i, h}, c_h, \cdot)$ is a prescription given some $\omega_{i, h}$ and $c_h$. We will define $\pi_i$ as a sequence of policies for agent $i$ at all steps $h\in[H]$, i.e., $\pi_i = (\pi_{i, 1}, \cdots, \pi_{i, H})$. A (potentially correlated) joint policy 
%\kz{reminder: do we have a notation for the ``space''  of such policies? I did not see it here, but will we use it later?}
is denoted as $\pi=\pi_1\odot\pi_2\cdots\odot\pi_n\in \Pi$.
%\kz{or at least we should say which space  does this $\pi_1\odot\pi_2\cdots\odot\pi_n$ belong to?}
 A \emph{product} policy is denoted as $\pi=\pi_1\times\pi_2\cdots\times\pi_n\in \Pi$ if {the distributions of drawing each seed $\omega_{i, h}$ for different agents are independent}. For Dec-POMDPs, using stochastic policies will not yield better policies than using only deterministic policies \citep{oliehoek2016concise}. 
%{For any policy $\pi\in\Delta(\Pi^{\mathrm{gen}})$  and event $\cE$, we write $\PP^{\cG}_{s_{1:h}, a_{1:h-1}, o_{2:h}\sim \pi_{1:h-1}}(\cE)$ to denote the probability of $\cE$ when $(s_{1:h},a_{1:h-1},o_{2:h})$ is drawn from a trajectory following the policy $\pi_{1:h-1}$ from step $1$ to $h-1$ in the model $\cG$. We will use the shorthand notation $\PP_{h}^{\pi_{1:h-1}, \cG}(\cdot)$ if the definition of $(s_{1:h},a_{1:h-1},o_{2:h})$ is evident. At times, if the time index $h$ is evident, we will write it as $\PP^{\pi, \cG}_{h}(\cdot)$. If the event $\cE$ does not depend on the choice of $\pi$, we will use $\PP_{h}^{\cG}(\cdot)$ and omit $\pi$. Similarly, we will write $\EE_{s_{1:h}, a_{1:h-1}, o_{2:h}\sim \pi}^\cG[\cdot]$ to denote expectations and use the shorthand notation $\EE^\cG[\cdot]$ if the expectation does not depend on the choice of $\pi$. Furthermore, if we are given some model $\cM$ (other than $\cG$), 
%\kz{NEW: to be clear, does this include a ``Markov game'' model (not a POSG model)? if so, are we sure this definition can be extended directly?}, 
%the notation of $\PP_{h}^\cM(\cdot)$, $\EE^{\cM}[\cdot]$ is defined in the same way.} We will hereafter use \emph{strategy} and  \emph{policy} interchangeably. 
% For simplicity of notations, we define the state visitation $d_{\cS, h}^{\cG, \pi}(s_h):=\PP_{h}^{\pi, \cG}(s_h)$}   

We are now ready to define the \emph{value function} for each agent:
\begin{definition}[Value function]\label{def:g_value_functioin}
For each agent $i\in [n]$ and step $h\in [H]$, given common information $c_h$ and joint policy  ${\pi}=\{\pi_{i}\}_{i=1}^{n}\in\Pi$, the 
\emph{value function {conditioned on the common information}} of agent $i$ is defined as: 
    $V^{{\pi}, \cG}_{i, h}(c_h) \vcentcolon= \EE_{\pi}^\cG\left[\sum_{h^{\prime}=h+1}^{H+1}r_{i, h^{\prime}}(o_{h^\prime})\biggiven c_{h}\right]$, where the expectation   is taken over the randomness from the model $\cG$, policy $\pi$, and the random seeds. For any $ c_{H+1}\in \cC_{H+1}: V^{{\pi}, \cG}_{i, H+1}(c_{H+1}) \vcentcolon= 0$.  {From now on, we will refer to  it as \emph{value function}  for short.} 
\end{definition} 

Another key concept in our analysis is the belief about the state \emph{and} the private information conditioned on the common information among agents. Formally, at step $h$, given policies from $1$ to $h-1$, we consider the common-information-based conditional belief $\PP^{{\pi}_{1:h-1}, \cG}_h\left(s_h, p_h\given c_h\right)$. This belief not only infers  the current underlying state $s_h$, but also each agent's private information $p_h$. With the common-information-based conditional belief, the value function given in Definition \ref{def:g_value_functioin}  has the following recursive structure: 
\begin{align}\label{dp}
    V^{{\pi}, \cG}_{i, h}(c_h) = \EE_{\pi}^{\cG}[r_{i, h+1}(o_{h+1}) + V^{{\pi}, \cG}_{i, h+1}(c_{h+1})\given c_h], 
\end{align} 
where the expectation is taken over the randomness of $(s_h,p_h,a_h,o_{h+1})$ given $\pi$.
With this relationship, we can define the \emph{prescription-value}  function correspondingly, a generalization of the \emph{action-value}  function in Markov games and MDPs, as follows.

\begin{definition}[Prescription-value function]\label{def:pres_value}
At step $h$, given the common information $c_h$, joint policies ${\pi}=\{\pi_{i}\}_{i=1}^{n}\in\Pi$, and prescriptions $\{\gamma_{i, h}\}_{i=1}^{n}\in\Gamma_h$, the \emph{prescription-value function  {conditioned on the common information and joint prescription}} of the $i^{th}$ agent is defined as: 
\begin{align*}
    &Q^{{\pi}, \cG}_{i, h}(c_h, \{\gamma_{j, h}\}_{j\in [n]}):= \EE_{\pi}^\cG\big[r_{i, h+1}(o_{h+1}) + V^{{\pi}, \cG}_{i, h+1}(c_{h+1})\Biggiven c_h, \{\gamma_{j, h}\}_{j\in [n]}\big],
\end{align*} 
where  prescription $\gamma_{i, h}\in \Delta(\cA_i)^{P_{i, h}}$ replaces the partial function $\pi_{i, h}(\cdot\given \omega_{i, h}, c_h, \cdot)$ in the value function. {From now on, we will refer to  it as \emph{prescription-value function}  for short.} 
\end{definition}
This prescription-value function indicates the expected return for {the $i^{th}$ agent} when all the agents firstly adopt the prescriptions $\{\gamma_{j, h}\}_{j\in [n]}$ and then follow the policy $\pi$. 


\subsection{Equilibrium notions}


With the definition of the value functions, we can accordingly define the solution concepts. Here we define the notions of  $\epsilon$-NE, $\epsilon$-CCE, $\epsilon$-CE, and $\epsilon$-team optimum {under the information-sharing framework}  
as follows. 

%\vspace{-3pt}
\begin{definition}[$\epsilon$-approximate Nash equilibrium {with information sharing}]
For any $\epsilon\ge 0$, a product policy $\pi^{\star}\in\Pi$ is an $\epsilon$-approximate Nash equilibrium  of the POSG $\cG$ with information sharing if:
\begin{align*}
    \operatorname{NE-gap}(\pi^\star):=\max_i \left(\max_{\pi_{i}^{\prime}\in \Pi_i}v_i^{\cG}(\pi_i^{\prime}\times {\pi^{\star}_{-i}})-v_i^{\cG}(\pi^\star)\right)\le  \epsilon.
\end{align*}
\end{definition}

\begin{definition}[$\epsilon$-approximate coarse correlated equilibrium {with information sharing}]
For any $\epsilon\ge 0$, a joint policy $\pi^{\star}\in\Pi$
%\kz{where was this $\Pi$ defined? does it mean product policy only or not?}
is an $\epsilon$-approximate coarse correlated equilibrium of the POSG $\cG$ with information sharing if:
\begin{align*}
    \operatorname{CCE-gap}(\pi^\star):=\max_i \left(\max_{\pi_{i}^{\prime}\in \Pi_i}v^{\cG}_{i}(\pi_i^{\prime}\times {\pi^{\star}_{-i}})-v_i^{\cG}(\pi^\star)\right)\le  \epsilon.
\end{align*}
\end{definition}

\begin{definition}[$\epsilon$-approximate correlated equilibrium {with information sharing}]\label{def:CCE}
For any $\epsilon\ge 0$, a joint policy $\pi^{\star}\in\Pi$ is an $\epsilon$-approximate correlated equilibrium of the POSG $\cG$ with information sharing if: 
\begin{align*}
    \operatorname{CE-gap}(\pi^\star):=\max_i \left(\max_{\phi_i}v_{i, 1}^{\cG}((\phi_i\diamond \pi_i^\star)\odot {\pi^{\star}_{-i}})-v_i^{\cG}(\pi^\star)\right)\le  \epsilon,
\end{align*} 
where $\phi_i$ is called \emph{strategy modification} and $\phi_i = \{\phi_{i, h, c_h, p_{i, h}}\}_{h, c_h, p_{i, h}}$, with  each $\phi_{i, h, c_h, p_{i, h}}:\cA_i\rightarrow \cA_i$ being a mapping from the action set to itself. The space of $\phi_i$ is denoted as $\Phi_i$. The composition $\phi_i\diamond\pi_i$ will work as follows: at the step $h$, when the agent $i$ is given $c_h$ and $p_{i, h}$, the action chosen to be $(a_{1, h}, \cdots, a_{i, h}, \cdots,a_{n, h})$ will be modified to $(a_{1, h}, \cdots, \phi_{i, h, c_h, p_{i, h}}(a_{i, h}), \cdots, a_{n, h})$. Note  that this definition follows from that in \cite{song2021can,liu2021sharp,jin2021v} when there exists common information, and is a natural generalization of the definition in the normal-form game case  \citep{roughgarden2010algorithmic}.
\end{definition} 
\subsection{Strategy independence of belief and examples}\label{subsec:example}
Here we take the examples from \cite{liu2023partially} to illustrate the generality of the information-sharing framework.

\begin{example}[One-step delayed 
sharing] At any step $h\in[H+1]$, the common and private information are  given as $c_h = \{o_{2:h-1}, a_{1:h-1}\}$ and $p_{i, h} = \{o_{i, h}\}$, respectively. In other words, the players  share all the action-observation history until the previous step $h-1$, with only the new observation being the private information. This model has been shown useful for power control \citep{altman2009stochastic}.
\end{example}  

\begin{example}[State controlled by one controller with asymmetric delay sharing] We assume there are $2$ players for convenience. It extends naturally to $n$-player settings. Consider the case where the state dynamics are controlled by player $1$, i.e., $\TT_h(\cdot\given s_h, a_{1, h}, a_{2, h}) = \TT_{h}(\cdot\given s_h, a_{1, h}, a_{2, h}^\prime)$ for all $s_h, a_{1, h}, a_{2, h}, a_{2, h}^\prime, h$. {There are two kinds of delay-sharing structures we could consider:} \textbf{Case A:} the information structure is given as $c_{h} = \{o_{1, 2:h}, o_{2, 2:h-d}, a_{1, 1:h-1}\}$, $p_{1, h} = \emptyset$, $p_{2, h} = \{ o_{2, h-d+1:h}\}$, i.e., player $1$'s observations are available to player $2$ instantly, while player $2$'s observations are available to player $1$ with a delay of $d\ge 1$ time steps. \textbf{Case B:} similar to \textbf{Case A} but player $1$'s observation is available to player $2$ with a delay of $1$ step. The information structure is given as $c_{h} = \{o_{1, 2:h-1}, o_{2, 2:h-d}, a_{1, 1:h-1}\}$, $p_{1, h} = \{o_{1, h}\}$, $p_{2, h} = \{ o_{2, h-d+1:h}\}$, where $d\ge 1$. This kind of asymmetric sharing is common in  network routing \citep{pathak2008measurement}, {where packages arrive at different hosts with different delays, leading to asymmetric delay sharing among hosts.} 
\end{example} 

\begin{example}[Symmetric information game] Consider the case when all observations and actions are available for all the agents, and there is no private information. Essentially, we have $c_h = \{o_{2:h}, a_{1:h-1}\}$ and $p_{i, h} = \emptyset$. We will also denote this structure  as \emph{fully sharing}  hereafter.	
\end{example}

\begin{example}[Information sharing with one-directional-one-step delay] Similar to the previous cases, we also assume there are $2$ players for ease of exposition,  and the case can be generalized to multi-player cases straightforwardly. Similar to the one-step delay case, we consider the situation where all observations of player $1$ are available to player $2$, while the observations of player $2$ are available to player $1$ with one-step delay. All past actions are available to both players. That is, in this case, $c_{h} = \{o_{1, 2:h}, o_{2,2:h-1}, a_{1:h-1}\}$, and player $1$ has no private information, i.e., $p_{1, h} =\emptyset$, and player $2$ has private information  $p_{2, h} = \{o_{2, h}\}$.
\end{example} 

\begin{example}[Uncontrolled state process] Consider the case where the state transition does not depend on the actions, that is, $\TT_h(\cdot\mid s_h, a_h) = \TT_h(\cdot\mid s_h, a_h^{\prime})$ for any $s_h, a_h, a_h^{\prime}, h$. 
    {Note that the agents are still coupled through the joint {reward}.}
    An example of this case is the information structure where controllers share their observations with a delay of $d\ge 1$ time steps. In this case, the common information is $c_h = \{o_{2:h-d}\}$ and the private information is $p_{i, h} = \{o_{i, h-d+1:h}\}$. {Such information structures {can be used to model} repeated games with incomplete information.}
\end{example}
It is worth mentioning that all previous examples satisfy the following important assumption and in the later discussion we will assume Assumption \ref{str_indi} holds.
\begin{assumption}[Strategy independence of beliefs]\label{str_indi}
Consider any step $h\in[H]$, any choice of joint policies ${\pi}\in\Pi$, and any realization of common information $c_h$ that has a non-zero probability under the trajectories generated by ${\pi}_{1:h-1}$. Consider any other policies ${\pi}^{\prime}_{1:h-1}$, which also give a non-zero probability to $c_h$. Then, we assume that: for any {such} $c_h\in\cC_h$, {and any} $p_{h}\in\cP_h, s_h\in \cS$, 
    $\PP^{{\pi}_{1:h-1}, \cG}_{h}\left(s_h, p_{h}\given c_h\right) = \PP^{{\pi}^{\prime}_{1:h-1}, \cG}_{h}\left(s_h, p_{h}\given c_h\right).$
\end{assumption}  

\section{Learning in POSG with asymmetric information}
\subsection{Reward-free learning of POSG}\label{subsec:posg-learn}
\begin{algorithm}[!h]
\begin{algorithmic}
\caption{Learning POSG\label{alg:eq-learn}}
\State  \textbf{Input:} $\cG, \text{Compress}_{1:H}$
\State $\hat{\cG}\leftarrow \text{Reward\_free}(\cG)$
\State $\{\PP^{\hat{\cM}}_h(\cdot, \cdot\given \hat{c}_h)\}_{h\in[H]}\leftarrow \text{Construct\_Belief}(\hat{\cG})$
\State Define the Markov game $\hat{\cM}$ using $\hat{\cG}$ and $\{\PP^{\hat{\cM}}_h(\cdot, \cdot\given \hat{c}_h)\}_{h\in[H]}$ as in \S\ref{subsec:posg-learn}
\State $\hat{\pi}\leftarrow\text{Common\_Information\_based\_Planning}(\hat{\cM})$ (see Algorithm 3 of \cite{liu2023partially})
\State \Return $\hat{\pi}$
\end{algorithmic}
\end{algorithm}

Our algorithm for POSG is similar to that for POMDP. We first learn an approximate POMDP and then construct an approximate Markov game where the state is \emph{compressed common information} and the action is the prescription. Specifically, we assume there exists a compressed common information space $\hat{\cC}_h$ and compression function $\text{Compress}_h:\cC_h\rightarrow\hat{\cC}_h$ such that we denote $\hat{c}_h:=\text{Compress}(c_h)$ for each $h\in[H]$. Meanwhile, we additionally assume the compressed common information evolves according to some function $\hat{\phi}_h$ such that $\hat{c}_{h+1}=\hat{\phi}_h(\hat{c}_h, \chi_{h+1}(p_h, a_h, o_{h+1}))$. Then given an approximate common information-based belief, i.e., $\PP_{h}^{\hat{\cM}}(s_h, p_h\given \hat{c}_h)$, we can define a Markov game $\hat{\cM}$ with state space $\hat{\cC}_{1:H}$, action space $\Gamma_{1:H}$, and the transition and rewards are defined according to
\$
\PP_h^{\hat{\cM}}&(\hat{c}_{h+1}\given \hat{c}_h, \gamma_h):=\\
&\sum_{s_h, p_h, a_h, s_{h+1}, o_{h+1}}\PP_{h}^{\hat{\cM}}(s_h, p_h\given \hat{c}_h)\prod_{i}\gamma_{i, h}(a_{i, h}\given p_{i, h})\hat{\TT}_{h}(s_{h+1}\given s_h, a_h)\hat{\OO}_{h+1}(o_{h+1}\given s_{h+1})\mathbbm{1}[\hat{c}_{h+1}=\hat{\phi}_{h}(\hat{c}_h, \chi_{h+1}(p_h, a_h, o_{h+1}))].
\$
\$
r_{i, h}^{\hat{\cM}}(\hat{c}_h, \gamma_h):=\EE_{s_{h}, p_{h}\sim \PP_{h}^{\hat{\cM}}(s_h, p_h\given \hat{c}_h)}\EE_{a_{i, h}\sim\gamma_{i, h}(\cdot\given p_{i, h})}[r_{i, h}(s_h, a_h)].
\$
Similar to Theorem \ref{lem:error}, we provide the error bound for the equilibrium solution of $\hat{\cM}$ in $\cG$.
\begin{theorem}\label{lem:error-posg}
	For $\hat{\cP}$ of Algorithm \ref{alg:reward-free-pomdp}, we define  
	\$
	\epsilon_{model}:&=\max_{\pi\in\Pi}\EE_{\pi}^\cP\sum_{h}\|\TT_{h}(\cdot\given s_h, a_h)-\hat{\TT}_{h}(\cdot\given s_h, a_h)\|_1+\|\OO_{h}(\cdot\given s_h)-\hat{\OO}_{h}(\cdot\given s_h)\|_1\\
	\epsilon_{belief}:&=\max_{\pi\in\Pi, h\in[H]}\EE_{\pi}^\cP\sum_{s_h, p_h}|\PP_h^{\cG}(s_h, p_h\given c_h)-\PP^{\hat{\cM}}_h(s_h, p_h\given \hat{c}_h)|.
	\$
	It holds that 
	\$
	\text{NE/CE/CCE-gap}(\hat{\pi}) \le 2(H\epsilon_{model}+H^2\epsilon_{belief}).
	\$
\end{theorem}	

\begin{proof}
	Consider any policy $\pi$, we here evaluate
	\$
	\EE_{\pi}^{\cG}&|V_{i, h}^{\pi, \cG}(c_h)-V_{i, h}^{\pi, \hat{\cM}}(c_h)|\\
	&=\EE_{\pi}^{\cG}|\EE_{\omega_{1:n, h}}[\EE_{s_h, p_h\sim\PP_h^{\cG}(\cdot, \cdot\given c_h), a_{j, h}\sim \pi_{j, h}(\cdot\given c_h, p_{j, h}, \omega_{j, h}), s_{h+1}\sim\TT_{h}(\cdot\given s_h, a_h), o_{h+1}\sim\OO_{h+1}(\cdot\given s_{h+1})}[r_{i, h}(s_h, a_h) + V_{i, h}^{\pi, \cP}(c_{h+1})]\\
	&-\EE_{s_h, p_h\sim\PP_h^{\hat{\cM}}(\cdot, \cdot\given \hat{c}_h), a_{j, h}\sim \pi_{j, h}(\cdot\given c_h, p_{j, h}, \omega_{j, h}), s_{h+1}\sim\hat{\TT}_{h}(\cdot\given s_h, a_h), o_{h+1}\sim\hat{\OO}_{h+1}(\cdot\given s_{h+1})}[r_{i, h}(s_h, a_h) + V_{i, h}^{\pi, \hat{\cM}}(c_{h+1})]]|\\
	&\le (H-h)\EE_{\pi}^\cG\sum_{\omega_{1:n, h}, s_h, p_h, a_h, s_{h+1}, o_{h+1}}|\PP_h(\omega_{1:n, h})\PP_h^\cG(s_h, p_h\given c_h)\prod_j\pi_{j, h}(a_{j, h}\given c_h, p_{j, h}, \omega_{j, h})\TT_h(s_{h+1}\given s_h, a_h)\OO_{h+1}(o_{h+1}\given s_{h+1})\\
	&\quad\quad-\PP_h(\omega_{1:n, h})\PP_h^{\hat{\cM}}(s_h, p_h\given c_h)\prod_j\pi_{j, h}(a_{j, h}\given c_h, p_{j, h}, \omega_{j, h})\hat{\TT}_h(s_{h+1}\given s_h, a_h)\hat{\OO}_{h+1}(o_{h+1}\given s_{h+1})| \\
	&\quad\quad + \EE_{\pi}^\cG |V_{i, h+1}^{\pi, \cG}(c_{h+1})-V_{i, h+1}^{\pi, \hat{\cM}}(c_{h+1})|\\
	&\le (H-h)\EE_{\pi}\|\TT_{h}(\cdot\given s_h, a_h)-\hat{\TT}_{h}(\cdot\given s_h, a_h)\|_1+\|\OO_{h}(\cdot\given s_h)-\hat{\OO}_{h+1}(\cdot\given s_{h+1})\|_1+\sum_{s_h, p_h}|\PP_h^{\cG}(s_h, p_h\given c_h)-\PP^{\hat{\cM}}_h(s_h, p_h\given \hat{c}_h)|\\
	&\quad\quad+\EE_{\pi}^\cG |V_{i, h+1}^{\pi, \cG}(c_{h+1})-V_{i, h+1}^{\pi, \hat{\cM}}(c_{h+1})|,
	\$
	where the first inequality comes from using Lemma \ref{lem:trick} repeatedly. By telescoping for $h=1$ to $H$, we conclude that
	\$
	|v_{i}^{\cG}(\pi)-v_{i}^{\hat{\cM}}(\pi)|\le H\epsilon_{model}+H^2\epsilon_{belief}.
	\$
	Therefore, for learning NE/CCE, for any $\pi_i\in\Pi_i$, it holds that
	\$
	v_{i}^{\cG}(\pi_i\times\hat{\pi}_{-i})-v_{i}^{\cG}(\hat{\pi})\le v_{i}^{\hat{\cM}}(\pi_i\times\hat{\pi}_{-i})-v_{i}^{\hat{\cM}}(\hat{\pi})+2(H\epsilon_{model}+H^2\epsilon_{belief})\le 2(H\epsilon_{model}+H^2\epsilon_{belief}),
	\$
	where the last step comes from Lemma \ref{lem:eq-m}, concluding that
	\$
	\text{NE/CCE-gap}(\hat{\pi})\le 2(H\epsilon_{model}+H^2\epsilon_{belief}).
	\$
	Similarly, for learning CE, for any strategy modification $\phi_i\in\Phi_i$, it holds that
	\$
	v_{i}^{\cG}((\phi_i\diamond\hat{\pi}_i)\odot\hat{\pi}_{-i})-v_{i}^{\cG}(\hat{\pi})\le v_{i}^{\hat{\cM}}((\phi_i\diamond\hat{\pi}_i)\odot\hat{\pi}_{-i})-v_{i}^{\hat{\cM}}(\hat{\pi})+2(H\epsilon_{model}+H^2\epsilon_{belief})\le 2(H\epsilon_{model}+H^2\epsilon_{belief}),
	\$
	where the last step comes from Lemma \ref{lem:eq-m}, concluding that
	\$
	\text{CE-gap}(\hat{\pi})\le 2(H\epsilon_{model}+H^2\epsilon_{belief}).
	\$
\end{proof}
With this theorem, we are ready to prove the sample and computation complexity of Algorithm \ref{alg:eq-learn} for learning the POSG.
\begin{theorem}\label{thm:posg-main}
		Fix $\epsilon, \delta>0$. Under Assumption \ref{assump:observa} and \ref{str_indi}, Algorithm \ref{alg:eq-learn} can learn an $\epsilon$-NE if $\cG$ is zero-sum or cooperative and $\epsilon$-CE/CCE if $\cG$ is general-sum with probability $1-\delta$ with sample complexity $\tilde{\cO}(\frac{S^2AHO+S^3AH}{\epsilon^2}+\frac{S^4A^2H^5}{\epsilon})$ and computation complexity $\max_{h\in[H]}\hat{C}_h\cdot\operatorname{poly}(S, A, P_h, H, \frac{1}{\epsilon_e})$. In particular, for examples in \S\ref{subsec:example}, the computation complexity is $(AO)^{\cO(\gamma^{-4}\log\frac{SH}{\epsilon})}$.
\end{theorem}
\begin{proof}
	By combing Theorem \ref{lem:free} and \ref{lem:error-posg}, it is guaranteed that Algorithm \ref{alg:eq-learn} can learn an $\epsilon$-NE if $\cG$ is zero-sum or cooperative and $\epsilon$-CE/CCE if $\cG$ is general-sum. Furthermore, the computation complexity is by Theorem 6 and 7 of \cite{liu2023partially}.
\end{proof}
We provide a supporting lemma below.
%We firstly point out some properties of the planning algorithm in $\hat{\cM}$.

\begin{lemma}[\cite{liu2023partially}]\label{lem:eq-m}
	Given $\hat{\cM}$, for computing NE/CCE, the output of Algorithm \ref{alg:eq-plan} satisfies that for any $h\in[H+1]$, $c_h\in\cC_h$, $\pi_i\in\Pi_i$
	\$
		V_{i, h}^{\pi_i\times\hat{\pi}_{-i}, \cM}(c_h)\le V_{i, h}^{\hat{\pi}, \cM}(c_h).
	\$ 
	For computing CE, the output of Algorithm \ref{alg:eq-plan} satisfies that for any $h\in[H+1]$, $c_h\in\cC_h$, $\phi_i\in\Phi_i$
	\$
		V_{i, h}^{(\phi_i\diamond\hat{\pi}_i)\odot\hat{\pi}_{-i}, \cM}(c_h)\le V_{i, h}^{\hat{\pi}, \cM}(c_h).
	\$ 

\end{lemma}

==> Body/UCB-VI.tex <==
\section{UCB-VI in POMDP}\label{sec:pomdp}

\begin{algorithm}[!h]
\begin{algorithmic}
\caption{Optimistic finite-memory value iteration\label{alg:ucbvi}}

\State  \textbf{Input:} $\cP$
\For{$k=1, 2, \cdots, K$}
	\For{$h\leftarrow H, H-1, \cdots, 1$}
		\For{$z_h\in\cZ_h$, $s_h\in\cS$}
			\State Define $Q_{h}^{\star, \cmk}(s_h, z_h, a_h):= r_{h}(s_h, a_h) + u_h^k(s_h, a_h)+ \EE_{s_{h+1}\sim \TT_h^k(\cdot\given s_h, a_h), o_{h+1}\sim\OO_{h+1}^k(\cdot\given s_{h+1})}[V_{h+1}^{\star, \cmk}(s_{h+1}, z_{h+1})]$
			\State Define $Q_{h}^{\star, \cmk}(z_h, a_h):= \EE_{s_h\sim b^{\cmk}_h(z_h)}[Q_{h}^{\star, \cmk}(s_h, z_h, a_h)]$
			\State $\pi^{k}_h(z_h) \leftarrow\argmax_{a_h\in\cA}Q_{h}^{\star, \cmk}(z_h, a_h)$
			\State $V_{h}^{\star, \cmk}(s_h, z_h)\leftarrow Q_{h}^{\star, \cmk}(s_h, z_h, \pi^{k}_h(z_h))$
		\EndFor		
	\EndFor
	\For{$h\in[H], s_h\in\cS, s_{h+1}\in\cS, a_h\in\cA, o_h\in\cO$}
		\State Execute $\pi^k$ and get trajectory $\tau^k=(s_{1:H}^k, a_{1:H}^k, o_{1:H}^k)$
		\State $N_{h}^{k+1}(s_h, a_h, s_{h+1})\leftarrow \sum_{l\in[k]}\mathbbm{1}[s_{h}^l = s_h, a_{h}^{l}=a_h, s_{h+1}^l = s_{h+1}]$
		\State $N_{h}^{k+1}(s_h, a_h)\leftarrow \sum_{l\in[k]}\mathbbm{1}[s_{h}^l = s_h, a_{h}^{l}=a_h]$
		\State $N_{h}^{k+1}(s_h, o_h)\leftarrow \sum_{l\in[k]}\mathbbm{1}[s_{h}^l = s_h, o_{h}^{l}=o_h]$
		\State $N_{h}^{k+1}(s_h)\leftarrow \sum_{l\in[k]}\mathbbm{1}[s_{h}^l = s]$
		\State $\TT^{k+1}_h(s_{h+1}\given s_h, a_h)\leftarrow \frac{N_{h}^{k+1}(s_h, a_h, s_{h+1})}{N_{h}^{k+1}(s_h, a_h)}$
		\State $\OO^{k+1}_h(o_{h}\given s_h)\leftarrow \frac{N_{h}^{k+1}(s_h, o_h)}{N_{h}^{k+1}(s_h)}$ 
		\State $r_{h}^{k+1}(s_h, a_h)\leftarrow r_{h}(s_h, a_h) + b_h^{k+1}(s_h, a_h)$ 	
	\EndFor
	\State Define ${\cP}^{k+1}:=(H, \cS, \cA, \cO, \{\TT^{k+1}_{h}\}_{h\in[H]}, \{\OO^{k+1}_h\}_{h\in[H]}, \mu_1, \{r_{h}^{k+1} + u_{h}^{k+1}\}_{h\in[H]})$ and its finite-memory MDP approximation ${\cM}^{k+1}$ accordingly.
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{lemma}[Optimism]
	With probability $1-2\delta$, for any $k\in[K]$, it holds that
	\$
	v^{\cmk}(\pi^k)\ge v^{\cP}(\pi^\star)
	\$

%	\$
%	v^{\cmk}(\pi^k)\ge \max_{\pi\in\Pi_L}v^{\cM}(\pi)
%	\$
\end{lemma}
\begin{proof}
	Consider any $\pi\in\Pi_L$, it holds that
	\$
		v^{\cmk}(\pi)- v^{\cP}(\pi)=\sum_h\EE_{\pi}^{\cP}[\EE_{s_{h+1}\sim \TT_{h}(\cdot\given \cdot, a_h)b_{h}(\tau_h)}^{\cP}[r_{h+1}(s_{h+1}, a_{h+1}) + Q_{h+1}^{\pi, \cmk}(s_{h+1}, o_{h+1}, a_{h+1})]-Q_{h}^{\pi, \cmk}(z_h, a_h)]
	\$
	Note that 
	\$
	Q_{h}^{\pi, \cmk}(s_h, z_h, a_h) = 
	\$
\end{proof}
\begin{proof}
	It suffices to prove that for any $\pi\in\Pi_L$ that $v^{\cmk}(\pi)\ge v^{\cM}(\pi)$.
	\$
	v^{\cmk}(\pi)- v^{\cM}(\pi)&=\EE_{\pi}^{\cmk}[\sum_{h}b_h^{\cmk}(z_h)^\top (r_h+u_h^k)(\cdot, a_h)]-\EE_{\pi}^{\cM}[\sum_{h}b_h^{\cM}(z_h)^\top r_h(\cdot, a_h)]\\
	&\ge \EE_{\pi}^{\cmk}[\sum_{h}b_h^{\cmk}(z_h)^\top (r_h+u_h^k)(\cdot, a_h)]-\EE_{\pi}^{\cmk}[\sum_{h}b_h^{\cM}(z_h)^\top r_h(\cdot, a_h)]-H\sum_{\tau}\|\PP^{\pi, \cM}(\tau)-\PP^{\pi, \cmk}(\tau)\|_1\\
	&\ge \EE_{\pi}^{\cmk}[\sum_{h}b_h^{\cmk}(z_h)^\top (r_h+u_h^k)(\cdot, a_h)]-\EE_{\pi}^{\cmk}[\sum_{h}b_h^{\cmk}(z_h)^\top r_h(\cdot, a_h) + \|b_h^{\cmk}(z_h)-b_h^{\cM}(z_h)\|_1]-H\sum_{\tau}\|\PP^{\pi, \cM}(\tau)-\PP^{\pi, \cmk}(\tau)\|_1\\
	&=\EE_{\pi}^{\cmk}[\sum_{h}b_h^{\cmk}(z_h)^\top u_h^k(\cdot, a_h) - \|b_h^{\cmk}(z_h)-b_h^{\cM}(z_h)\|_1]-H\sum_{\tau}\|\PP^{\pi, \cM}(\tau)-\PP^{\pi, \cmk}(\tau)\|_1
	\$
\end{proof}

\begin{lemma}
	Denote $\pi^\star\in\argmax_{\pi\in\Pi_{L}}v^{\cM}(\pi)$. We define
	\$
	\text{Regret}(K)=\sum_{k=1}^K \max_{\pi\in\Pi}v^{\cP}(\pi) - v^{\cP}(\pi^k).
	\$
	We have $\text{Regret}(K)\le$
\end{lemma}
\begin{proof}
	Note that for any $k\in[K]$, we have 
	\$
	\max_{\pi\in\Pi}v^{\cP}(\pi) - v^{\cP}(\pi^k)\le v^{\cM}(\pi^\star) - v^{\cP}(\pi^k)+\epsilon\le v^{\cmk}(\pi^k) - v^{\cP}(\pi^k)+\epsilon 
	\$
\end{proof}

